The dissimilar chemical composition of the planet-hosting stars of the XO-2 binary system

Using high-quality spectra of the twin stars in the XO-2 binary system, we have detected significant differences in the chemical composition of their photospheres. The differences correlate strongly with the elements' dust condensation temperature. In XO-2N, volatiles are enhanced by about 0.015 dex and refractories are overabundant by up to 0.090 dex. On average, our error bar in relative abundance is 0.012 dex. We present an early metal-depletion scenario in which the formation of the gas giant planets known to exist around these stars is responsible for a 0.015 dex offset in the abundances of all elements while 20 M_Earth of non-detected rocky objects that formed around XO-2S explain the additional refractory-element difference. An alternative explanation involves the late accretion of at least 20 M_Earth of planet-like material by XO-2N, allegedly as a result of the migration of the hot Jupiter detected around that star. Dust cleansing by a nearby hot star as well as age or Galactic birthplace effects can be ruled out as valid explanations for this phenomenon.

==> linelist.tex <==
5052.167 & 6.0 & 7.685 & -1.304 & 32.0 & 34.2 & 32.8 \\
6587.6099 & 6.0 & 8.537 & -1.021 & 10.8 & 12.1 & 13.8 \\
7111.469 & 6.0 & 8.64 & -1.074 & 17.7 & 19.1 & 10.7 \\
7116.96 & 6.0 & 8.65 & -0.91 & 11.9 & 12.7 & 13.2 \\
4218.723 & 106.0 & 0.413 & -1.008 & 92.5 & 93.9 & 79.5 \\
4253.003 & 106.0 & 0.523 & -1.523 & 43.3 & 44.3 & 33.3 \\
4253.209 & 106.0 & 0.523 & -1.486 & 42.2 & 43.8 & 33.8 \\
7771.9438 & 8.0 & 9.146 & 0.352 & 44.2 & 48.3 & 68.7 \\
7775.3901 & 8.0 & 9.146 & 0.002 & 38.9 & 42.0 & 48.0 \\
4751.8218 & 11.0 & 2.104 & -2.078 & 39.1 & 34.9 & 18.4 \\
4982.82 & 11.0 & 2.1 & -1.0 & 103.5 & 101.9 & 81.9 \\
5148.838 & 11.0 & 2.102 & -2.044 & 40.9 & 36.3 & 10.0 \\
5682.64 & 11.0 & 2.1 & -0.77 & 168.5 & 160.6 & 100.3 \\
5688.21 & 11.0 & 2.1 & -0.48 & 187.4 & 180.9 & 121.6 \\
6154.2251 & 11.0 & 2.102 & -1.547 & 92.7 & 87.9 & 36.4 \\
6160.7471 & 11.0 & 2.104 & -1.246 & 111.8 & 104.9 & 55.3 \\
4730.04 & 12.0 & 4.34 & -2.39 & 121.2 & 111.8 & 69.2 \\
5711.0879 & 12.0 & 4.345 & -1.729 & 155.8 & 148.5 & 104.9 \\
6318.717 & 12.0 & 5.108 & -1.945 & 95.2 & 86.1 & 37.3 \\
6319.2368 & 12.0 & 5.108 & -2.324 & 62.4 & 57.5 & 24.5 \\
5557.07 & 13.0 & 3.14 & -2.21 & 38.8 & 32.6 & 11.7 \\
6696.0181 & 13.0 & 3.143 & -1.481 & 85.7 & 79.5 & 38.1 \\
6698.667 & 13.0 & 3.143 & -1.782 & 63.2 & 53.4 & 21.2 \\
5488.983 & 14.0 & 5.614 & -1.69 & 40.4 & 35.5 & 20.2 \\
5517.54 & 14.0 & 5.08 & -2.496 & 27.2 & 25.1 & 12.7 \\
5645.6128 & 14.0 & 4.93 & -2.043 & 62.9 & 60.1 & 35.5 \\
5665.554 & 14.0 & 4.92 & -1.94 & 73.1 & 70.0 & 40.9 \\
5684.4839 & 14.0 & 4.954 & -1.553 & 82.4 & 80.0 & 60.2 \\
5690.4248 & 14.0 & 4.93 & -1.773 & 69.7 & 67.7 & 49.8 \\
5701.105 & 14.0 & 4.93 & -1.953 & 59.0 & 55.1 & 38.7 \\
5753.64 & 14.0 & 5.62 & -1.333 & 91.4 & 86.4 & 47.9 \\
5772.145 & 14.0 & 5.082 & -1.653 & 76.0 & 73.4 & 53.0 \\
5793.0732 & 14.0 & 4.93 & -1.963 & 65.5 & 63.4 & 43.0 \\
5797.87 & 14.0 & 4.95 & -1.912 & 79.7 & 72.4 & 43.0 \\
5948.54 & 14.0 & 5.08 & -1.208 & 111.3 & 107.5 & 86.2 \\
6125.03 & 14.0 & 5.61 & -1.51 & 54.5 & 51.3 & 32.3 \\
6142.49 & 14.0 & 5.62 & -1.54 & 50.6 & 48.5 & 31.9 \\
6145.02 & 14.0 & 5.61 & -1.48 & 59.4 & 57.5 & 38.5 \\
6155.14 & 14.0 & 5.62 & -0.72 & 117.0 & 108.9 & 79.6 \\
6195.46 & 14.0 & 5.87 & -1.666 & 36.8 & 34.5 & 17.4 \\
6237.33 & 14.0 & 5.61 & -1.116 & 94.8 & 91.3 & 60.3 \\
6243.82 & 14.0 & 5.62 & -1.31 & 72.6 & 64.6 & 45.1 \\
6244.48 & 14.0 & 5.61 & -1.36 & 71.9 & 68.7 & 43.8 \\
6414.98 & 14.0 & 5.87 & -1.08 & 71.7 & 66.7 & 46.9 \\
6527.21 & 14.0 & 5.87 & -1.227 & 71.5 & 66.0 & 37.7 \\
6721.84 & 14.0 & 5.863 & -1.06 & 78.1 & 73.0 & 43.3 \\
6741.64 & 14.0 & 5.984 & -1.653 & 31.9 & 31.5 & 15.9 \\
7226.206 & 14.0 & 5.614 & -1.413 & 87.7 & 80.5 & 39.6 \\
7405.77 & 14.0 & 5.614 & -0.72 & 116.6 & 115.3 & 90.2 \\
7415.96 & 14.0 & 5.61 & -0.85 & 100.2 & 100.6 & 87.0 \\
7423.52 & 14.0 & 5.62 & -0.65 & 117.4 & 116.5 & 98.6 \\
7760.64 & 14.0 & 6.2 & -1.37 & 22.8 & 23.5 & 15.3 \\
7800.0 & 14.0 & 6.18 & -0.71 & 82.8 & 76.9 & 54.6 \\
4694.1128 & 16.0 & 6.525 & -1.673 & 16.2 & 16.9 & 11.2 \\
4695.4429 & 16.0 & 6.525 & -1.829 & 12.7 & 13.1 & 7.8 \\
6052.656 & 16.0 & 7.87 & -0.4 & 16.9 & 16.9 & 10.9 \\
6743.54 & 16.0 & 7.866 & -0.6 & 6.9 & 7.5 & 8.4 \\
6757.1709 & 16.0 & 7.87 & -0.353 & 14.9 & 15.5 & 15.5 \\
7686.1602 & 16.0 & 7.868 & -1.013 & 7.5 & 8.1 & 3.8 \\
7698.9741 & 19.0 & 0.0 & -0.177 & 217.0 & 210.0 & 157.4 \\
4512.2681 & 20.0 & 2.526 & -1.901 & 55.5 & 49.5 & 21.8 \\
5260.3872 & 20.0 & 2.521 & -1.719 & 63.8 & 58.6 & 30.2 \\
5261.71 & 20.0 & 2.52 & -0.677 & 144.2 & 137.3 & 98.8 \\
5512.98 & 20.0 & 2.93 & -0.559 & 131.9 & 119.7 & 83.6 \\
5581.97 & 20.0 & 2.52 & -0.63 & 139.8 & 132.8 & 94.9 \\
5590.12 & 20.0 & 2.52 & -0.65 & 127.4 & 118.1 & 90.4 \\
5867.562 & 20.0 & 2.933 & -1.57 & 60.5 & 53.2 & 22.6 \\
6156.02 & 20.0 & 2.52 & -2.497 & 31.5 & 25.7 & 8.2 \\
6161.2969 & 20.0 & 2.523 & -1.266 & 106.3 & 99.0 & 61.4 \\
6163.755 & 20.0 & 2.521 & -1.286 & 102.0 & 96.0 & 63.0 \\
6166.439 & 20.0 & 2.521 & -1.142 & 111.3 & 104.4 & 69.5 \\
6169.042 & 20.0 & 2.523 & -0.797 & 143.0 & 133.3 & 92.0 \\
6169.55 & 20.0 & 2.52 & -0.58 & 166.6 & 156.1 & 112.4 \\
6449.82 & 20.0 & 2.52 & -0.733 & 147.0 & 137.6 & 101.5 \\
6455.5981 & 20.0 & 2.523 & -1.34 & 97.7 & 91.3 & 56.1 \\
6471.6621 & 20.0 & 2.526 & -0.686 & 134.0 & 126.3 & 90.6 \\
6499.6499 & 20.0 & 2.523 & -0.818 & 128.9 & 121.1 & 85.8 \\
6572.8 & 20.0 & 0.0 & -4.28 & 98.1 & 87.2 & 32.3 \\
4743.8208 & 21.0 & 1.448 & 0.422 & 44.8 & 35.7 & 8.6 \\
5081.561 & 21.0 & 1.448 & 0.469 & 45.4 & 36.1 & 7.4 \\
5520.5 & 21.0 & 1.87 & 0.562 & 28.3 & 25.3 & 6.6 \\
5671.8281 & 21.0 & 1.448 & 0.495 & 65.6 & 54.8 & 13.9 \\
5686.856 & 21.0 & 1.439 & 0.376 & 46.3 & 38.4 & 8.5 \\
5526.82 & 21.1 & 1.77 & 0.14 & 88.8 & 87.1 & 74.7 \\
5657.88 & 21.1 & 1.51 & -0.326 & 80.6 & 77.0 & 67.1 \\
5667.14 & 21.1 & 1.5 & -1.025 & 55.5 & 51.6 & 30.8 \\
5669.055 & 21.1 & 1.5 & -1.2 & 47.6 & 46.0 & 34.6 \\
5684.2139 & 21.1 & 1.507 & -1.074 & 51.6 & 49.8 & 37.2 \\
6245.6411 & 21.1 & 1.507 & -1.036 & 48.3 & 45.8 & 33.0 \\
6320.843 & 21.1 & 1.5 & -1.923 & 13.5 & 12.4 & 7.6 \\
6604.5781 & 21.1 & 1.357 & -1.309 & 56.1 & 52.0 & 35.5 \\
4512.733 & 22.0 & 0.84 & -0.42 & 101.4 & 94.6 & 66.5 \\
4518.023 & 22.0 & 0.83 & -0.27 & 111.8 & 104.8 & 71.2 \\
4555.485 & 22.0 & 0.85 & -0.43 & 99.2 & 92.3 & 63.1 \\
4562.64 & 22.0 & 0.02 & -2.6 & 53.5 & 45.9 & 12.1 \\
4617.28 & 22.0 & 1.75 & 0.45 & 99.0 & 93.4 & 62.9 \\
4623.1 & 22.0 & 1.74 & 0.17 & 101.5 & 91.9 & 59.0 \\
4645.19 & 22.0 & 1.73 & -0.666 & 58.4 & 52.1 & 22.9 \\
4656.47 & 22.0 & 0.0 & -1.308 & 104.1 & 97.6 & 67.0 \\
4675.11 & 22.0 & 1.07 & -0.939 & 83.6 & 77.8 & 38.6 \\
4722.61 & 22.0 & 1.05 & -1.433 & 64.9 & 56.6 & 18.2 \\
4758.118 & 22.0 & 2.249 & 0.481 & 74.1 & 69.1 & 42.5 \\
4759.269 & 22.0 & 2.256 & 0.57 & 77.8 & 72.8 & 45.9 \\
4778.258 & 22.0 & 2.236 & -0.22 & 51.8 & 45.7 & 16.2 \\
4820.41 & 22.0 & 1.5 & -0.39 & 83.9 & 76.9 & 43.5 \\
4840.88 & 22.0 & 0.9 & -0.45 & 100.4 & 95.1 & 65.6 \\
4858.14 & 22.0 & 4.102 & -0.14 & 35.3 & 26.7 & 7.7 \\
4913.616 & 22.0 & 1.87 & 0.22 & 87.2 & 83.5 & 51.5 \\
4964.715 & 22.0 & 1.969 & -0.82 & 36.7 & 28.9 & 8.6 \\
4997.1 & 22.0 & 0.0 & -2.174 & 79.5 & 72.5 & 32.7 \\
4999.5 & 22.0 & 0.83 & 0.27 & 156.1 & 142.6 & 101.8 \\
5016.162 & 22.0 & 0.85 & -0.52 & 101.9 & 95.5 & 65.6 \\
5022.866 & 22.0 & 0.826 & -0.378 & 115.9 & 106.9 & 71.2 \\
5024.85 & 22.0 & 0.818 & -0.56 & 115.6 & 108.0 & 71.0 \\
5039.96 & 22.0 & 0.02 & -1.199 & 121.7 & 114.3 & 76.5 \\
5064.06 & 22.0 & 2.69 & -0.471 & 24.3 & 19.9 & 5.8 \\
5071.49 & 22.0 & 1.46 & -0.797 & 80.1 & 72.8 & 29.4 \\
5087.06 & 22.0 & 1.43 & -0.78 & 85.4 & 75.1 & 27.6 \\
5113.439 & 22.0 & 1.443 & -0.727 & 67.2 & 63.0 & 27.7 \\
5145.459 & 22.0 & 1.46 & -0.518 & 77.5 & 71.3 & 35.0 \\
5147.477 & 22.0 & 0.0 & -1.956 & 80.8 & 74.9 & 38.7 \\
5152.184 & 22.0 & 0.021 & -1.968 & 79.9 & 73.9 & 36.0 \\
5186.33 & 22.0 & 2.117 & -0.77 & 27.3 & 21.3 & 4.9 \\
5192.97 & 22.0 & 0.02 & -0.99 & 130.6 & 121.3 & 83.4 \\
5210.38 & 22.0 & 0.05 & -0.85 & 139.7 & 128.1 & 89.9 \\
5219.699 & 22.0 & 0.021 & -2.236 & 82.0 & 74.5 & 27.7 \\
5223.62 & 22.0 & 2.092 & -0.49 & 45.8 & 41.5 & 14.6 \\
5224.304 & 22.0 & 2.134 & 0.13 & 77.3 & 73.1 & 41.1 \\
5247.288 & 22.0 & 2.103 & -0.64 & 36.4 & 30.1 & 5.9 \\
5252.098 & 22.0 & 0.048 & -2.392 & 66.6 & 59.4 & 19.5 \\
5295.774 & 22.0 & 1.067 & -1.577 & 48.2 & 42.0 & 12.8 \\
5299.98 & 22.0 & 1.05 & -1.47 & 56.0 & 48.9 & 20.3 \\
5426.26 & 22.0 & 0.02 & -2.95 & 44.7 & 35.4 & 6.9 \\
5471.2 & 22.0 & 1.44 & -1.4 & 42.3 & 34.9 & 8.8 \\
5474.23 & 22.0 & 1.46 & -1.23 & 48.6 & 40.0 & 10.9 \\
5474.46 & 22.0 & 2.34 & -0.85 & 18.4 & 14.8 & 3.5 \\
5490.147 & 22.0 & 1.46 & -0.877 & 62.9 & 56.6 & 21.3 \\
5503.9 & 22.0 & 2.58 & -0.218 & 50.1 & 40.3 & 12.4 \\
5648.57 & 22.0 & 2.49 & -0.41 & 39.9 & 33.1 & 10.4 \\
5662.147 & 22.0 & 2.318 & 0.01 & 56.1 & 50.3 & 22.9 \\
5689.459 & 22.0 & 2.297 & -0.36 & 47.6 & 40.4 & 13.4 \\
5702.658 & 22.0 & 2.292 & -0.59 & 33.6 & 26.3 & 6.4 \\
5716.441 & 22.0 & 2.297 & -0.72 & 33.2 & 25.6 & 7.1 \\
5737.07 & 22.0 & 1.06 & -0.815 & 61.7 & 50.3 & 10.8 \\
5739.464 & 22.0 & 2.249 & -0.6 & 34.5 & 27.4 & 8.5 \\
5766.33 & 22.0 & 3.29 & 0.326 & 34.6 & 29.3 & 9.0 \\
5866.452 & 22.0 & 1.066 & -0.84 & 102.0 & 91.7 & 48.7 \\
5953.17 & 22.0 & 1.89 & -0.27 & 78.0 & 70.8 & 33.5 \\
5965.84 & 22.0 & 1.88 & -0.492 & 69.1 & 60.1 & 25.1 \\
5978.55 & 22.0 & 1.87 & -0.602 & 65.1 & 58.8 & 23.9 \\
6064.63 & 22.0 & 1.05 & -1.941 & 44.6 & 37.4 & 8.6 \\
6091.18 & 22.0 & 2.267 & -0.37 & 51.3 & 44.0 & 14.3 \\
6126.217 & 22.0 & 1.066 & -1.424 & 68.3 & 61.3 & 22.8 \\
6258.099 & 22.0 & 1.443 & -0.299 & 92.2 & 85.9 & 51.1 \\
6261.101 & 22.0 & 1.429 & -0.479 & 104.0 & 92.7 & 48.6 \\
6303.753 & 22.0 & 1.443 & -1.51 & 40.3 & 33.8 & 8.1 \\
6312.234 & 22.0 & 1.46 & -1.496 & 41.3 & 32.6 & 7.9 \\
6599.104 & 22.0 & 0.9 & -2.029 & 49.1 & 39.5 & 9.4 \\
6743.13 & 22.0 & 0.899 & -1.63 & 71.1 & 60.3 & 18.2 \\
7949.15 & 22.0 & 1.5 & -1.46 & 49.1 & 42.0 & 12.1 \\
4409.5196 & 22.1 & 1.231 & -2.57 & 51.0 & 47.4 & 37.5 \\
4444.536 & 22.1 & 1.116 & -2.21 & 76.9 & 72.4 & 61.3 \\
4493.5225 & 22.1 & 1.08 & -2.83 & 38.9 & 36.8 & 34.2 \\
4583.4086 & 22.1 & 1.165 & -2.87 & 41.5 & 38.2 & 30.4 \\
4609.2653 & 22.1 & 1.18 & -3.43 & 21.6 & 19.0 & 12.6 \\
4636.32 & 22.1 & 1.165 & -3.02 & 29.5 & 26.3 & 19.2 \\
4657.212 & 22.1 & 1.243 & -2.32 & 57.3 & 55.5 & 48.5 \\
4708.6621 & 22.1 & 1.237 & -2.37 & 56.8 & 57.2 & 50.0 \\
4719.533 & 22.1 & 1.243 & -3.28 & 19.3 & 18.8 & 12.6 \\
4764.5237 & 22.1 & 1.237 & -2.77 & 43.1 & 40.6 & 32.9 \\
4798.5315 & 22.1 & 1.08 & -2.67 & 57.5 & 54.3 & 44.1 \\
4865.6114 & 22.1 & 1.116 & -2.81 & 56.0 & 50.5 & 40.8 \\
4874.014 & 22.1 & 3.095 & -0.8 & 40.9 & 39.4 & 36.1 \\
4911.2 & 22.1 & 3.12 & -0.61 & 63.4 & 60.9 & 51.9 \\
5005.16 & 22.1 & 1.566 & -2.72 & 34.5 & 32.8 & 20.2 \\
5154.08 & 22.1 & 1.57 & -1.75 & 99.3 & 94.6 & 70.6 \\
5185.91 & 22.1 & 1.89 & -1.49 & 63.0 & 60.5 & 61.2 \\
5211.53 & 22.1 & 2.59 & -1.16 & 39.3 & 37.9 & 32.4 \\
5418.7675 & 22.1 & 1.582 & -2.11 & 61.3 & 59.4 & 48.6 \\
5490.69 & 22.1 & 1.566 & -2.43 & 29.4 & 26.8 & 20.8 \\
6606.979 & 22.1 & 2.061 & -2.76 & 15.3 & 13.7 & 8.7 \\
4586.3418 & 23.0 & 0.0401 & -1.466 & 96.7 & 92.8 & 38.1 \\
-4586.353 & 23.0 & 0.0401 & -1.571 & 0.0 & 0.0 & 0.0 \\
-4586.3628 & 23.0 & 0.0401 & -1.687 & 0.0 & 0.0 & 0.0 \\
-4586.3652 & 23.0 & 0.0401 & -2.474 & 0.0 & 0.0 & 0.0 \\
-4586.3711 & 23.0 & 0.0401 & -1.816 & 0.0 & 0.0 & 0.0 \\
-4586.373 & 23.0 & 0.0401 & -2.263 & 0.0 & 0.0 & 0.0 \\
-4586.3779 & 23.0 & 0.0401 & -1.962 & 0.0 & 0.0 & 0.0 \\
-4586.3799 & 23.0 & 0.0401 & -2.19 & 0.0 & 0.0 & 0.0 \\
-4586.3838 & 23.0 & 0.0401 & -2.132 & 0.0 & 0.0 & 0.0 \\
-4586.3848 & 23.0 & 0.0401 & -2.184 & 0.0 & 0.0 & 0.0 \\
-4586.3848 & 23.0 & 0.0401 & -3.775 & 0.0 & 0.0 & 0.0 \\
-4586.3901 & 23.0 & 0.0401 & -2.231 & 0.0 & 0.0 & 0.0 \\
-4586.3901 & 23.0 & 0.0401 & -2.336 & 0.0 & 0.0 & 0.0 \\
-4586.3901 & 23.0 & 0.0401 & -3.377 & 0.0 & 0.0 & 0.0 \\
-4586.3931 & 23.0 & 0.0401 & -2.336 & 0.0 & 0.0 & 0.0 \\
-4586.394 & 23.0 & 0.0401 & -2.599 & 0.0 & 0.0 & 0.0 \\
-4586.394 & 23.0 & 0.0401 & -3.173 & 0.0 & 0.0 & 0.0 \\
-4586.395 & 23.0 & 0.0401 & -2.532 & 0.0 & 0.0 & 0.0 \\
-4586.397 & 23.0 & 0.0401 & -3.076 & 0.0 & 0.0 & 0.0 \\
-4586.3979 & 23.0 & 0.0401 & -3.076 & 0.0 & 0.0 & 0.0 \\
-4586.3989 & 23.0 & 0.0401 & -3.231 & 0.0 & 0.0 & 0.0 \\
4594.093 & 23.0 & 0.068 & -2.096 & 124.7 & 117.2 & 56.8 \\
-4594.096 & 23.0 & 0.068 & -2.548 & 0.0 & 0.0 & 0.0 \\
-4594.096 & 23.0 & 0.068 & -1.978 & 0.0 & 0.0 & 0.0 \\
-4594.101 & 23.0 & 0.068 & -3.548 & 0.0 & 0.0 & 0.0 \\
-4594.101 & 23.0 & 0.068 & -2.337 & 0.0 & 0.0 & 0.0 \\
-4594.101 & 23.0 & 0.068 & -1.86 & 0.0 & 0.0 & 0.0 \\
-4594.107 & 23.0 & 0.068 & -3.342 & 0.0 & 0.0 & 0.0 \\
-4594.107 & 23.0 & 0.068 & -2.241 & 0.0 & 0.0 & 0.0 \\
-4594.107 & 23.0 & 0.068 & -1.748 & 0.0 & 0.0 & 0.0 \\
-4594.115 & 23.0 & 0.068 & -3.313 & 0.0 & 0.0 & 0.0 \\
-4594.115 & 23.0 & 0.068 & -2.205 & 0.0 & 0.0 & 0.0 \\
-4594.115 & 23.0 & 0.068 & -1.644 & 0.0 & 0.0 & 0.0 \\
-4594.125 & 23.0 & 0.068 & -3.393 & 0.0 & 0.0 & 0.0 \\
-4594.125 & 23.0 & 0.068 & -2.221 & 0.0 & 0.0 & 0.0 \\
-4594.125 & 23.0 & 0.068 & -1.548 & 0.0 & 0.0 & 0.0 \\
-4594.136 & 23.0 & 0.068 & -3.585 & 0.0 & 0.0 & 0.0 \\
-4594.136 & 23.0 & 0.068 & -2.303 & 0.0 & 0.0 & 0.0 \\
-4594.136 & 23.0 & 0.068 & -1.458 & 0.0 & 0.0 & 0.0 \\
-4594.149 & 23.0 & 0.068 & -3.974 & 0.0 & 0.0 & 0.0 \\
-4594.149 & 23.0 & 0.068 & -2.521 & 0.0 & 0.0 & 0.0 \\
-4594.149 & 23.0 & 0.068 & -1.374 & 0.0 & 0.0 & 0.0 \\
4875.462 & 23.0 & 0.04 & -2.616 & 105.5 & 94.3 & 46.4 \\
-4875.464 & 23.0 & 0.04 & -2.331 & 0.0 & 0.0 & 0.0 \\
-4875.464 & 23.0 & 0.04 & -2.586 & 0.0 & 0.0 & 0.0 \\
-4875.468 & 23.0 & 0.04 & -2.586 & 0.0 & 0.0 & 0.0 \\
-4875.468 & 23.0 & 0.04 & -2.143 & 0.0 & 0.0 & 0.0 \\
-4875.468 & 23.0 & 0.04 & -2.637 & 0.0 & 0.0 & 0.0 \\
-4875.474 & 23.0 & 0.04 & -2.198 & 0.0 & 0.0 & 0.0 \\
-4875.474 & 23.0 & 0.04 & -2.052 & 0.0 & 0.0 & 0.0 \\
-4875.474 & 23.0 & 0.04 & -2.762 & 0.0 & 0.0 & 0.0 \\
-4875.481 & 23.0 & 0.04 & -1.943 & 0.0 & 0.0 & 0.0 \\
-4875.481 & 23.0 & 0.04 & -2.03 & 0.0 & 0.0 & 0.0 \\
-4875.481 & 23.0 & 0.04 & -2.984 & 0.0 & 0.0 & 0.0 \\
-4875.491 & 23.0 & 0.04 & -1.745 & 0.0 & 0.0 & 0.0 \\
-4875.491 & 23.0 & 0.04 & -2.084 & 0.0 & 0.0 & 0.0 \\
-4875.491 & 23.0 & 0.04 & -3.394 & 0.0 & 0.0 & 0.0 \\
-4875.503 & 23.0 & 0.04 & -1.581 & 0.0 & 0.0 & 0.0 \\
-4875.503 & 23.0 & 0.04 & -2.28 & 0.0 & 0.0 & 0.0 \\
-4875.517 & 23.0 & 0.04 & -1.44 & 0.0 & 0.0 & 0.0 \\
4881.499 & 23.0 & 0.0686 & -3.639 & 125.3 & 115.5 & 57.0 \\
-4881.5122 & 23.0 & 0.0686 & -2.338 & 0.0 & 0.0 & 0.0 \\
-4881.522 & 23.0 & 0.0686 & -3.241 & 0.0 & 0.0 & 0.0 \\
-4881.5259 & 23.0 & 0.0686 & -1.33 & 0.0 & 0.0 & 0.0 \\
-4881.5327 & 23.0 & 0.0686 & -2.127 & 0.0 & 0.0 & 0.0 \\
-4881.542 & 23.0 & 0.0686 & -3.037 & 0.0 & 0.0 & 0.0 \\
-4881.5459 & 23.0 & 0.0686 & -1.435 & 0.0 & 0.0 & 0.0 \\
-4881.5508 & 23.0 & 0.0686 & -2.054 & 0.0 & 0.0 & 0.0 \\
-4881.5591 & 23.0 & 0.0686 & -2.94 & 0.0 & 0.0 & 0.0 \\
-4881.562 & 23.0 & 0.0686 & -1.551 & 0.0 & 0.0 & 0.0 \\
-4881.5659 & 23.0 & 0.0686 & -2.048 & 0.0 & 0.0 & 0.0 \\
-4881.5728 & 23.0 & 0.0686 & -2.94 & 0.0 & 0.0 & 0.0 \\
-4881.5752 & 23.0 & 0.0686 & -1.68 & 0.0 & 0.0 & 0.0 \\
-4881.5781 & 23.0 & 0.0686 & -2.095 & 0.0 & 0.0 & 0.0 \\
-4881.584 & 23.0 & 0.0686 & -3.095 & 0.0 & 0.0 & 0.0 \\
-4881.585 & 23.0 & 0.0686 & -1.826 & 0.0 & 0.0 & 0.0 \\
-4881.5869 & 23.0 & 0.0686 & -2.2 & 0.0 & 0.0 & 0.0 \\
-4881.5928 & 23.0 & 0.0686 & -1.996 & 0.0 & 0.0 & 0.0 \\
-4881.5928 & 23.0 & 0.0686 & -2.396 & 0.0 & 0.0 & 0.0 \\
-4881.5972 & 23.0 & 0.0686 & -2.2 & 0.0 & 0.0 & 0.0 \\
-4881.5977 & 23.0 & 0.0686 & -2.463 & 0.0 & 0.0 & 0.0 \\
5670.832 & 23.0 & 1.08 & -3.402 & 81.7 & 70.9 & 19.9 \\
-5670.832 & 23.0 & 1.08 & -2.101 & 0.0 & 0.0 & 0.0 \\
-5670.832 & 23.0 & 1.08 & -1.093 & 0.0 & 0.0 & 0.0 \\
-5670.844 & 23.0 & 1.08 & -3.004 & 0.0 & 0.0 & 0.0 \\
-5670.844 & 23.0 & 1.08 & -1.891 & 0.0 & 0.0 & 0.0 \\
-5670.844 & 23.0 & 1.08 & -1.198 & 0.0 & 0.0 & 0.0 \\
-5670.854 & 23.0 & 1.08 & -2.8 & 0.0 & 0.0 & 0.0 \\
-5670.854 & 23.0 & 1.08 & -1.817 & 0.0 & 0.0 & 0.0 \\
-5670.854 & 23.0 & 1.08 & -1.314 & 0.0 & 0.0 & 0.0 \\
-5670.863 & 23.0 & 1.08 & -2.703 & 0.0 & 0.0 & 0.0 \\
-5670.863 & 23.0 & 1.08 & -1.811 & 0.0 & 0.0 & 0.0 \\
-5670.863 & 23.0 & 1.08 & -1.443 & 0.0 & 0.0 & 0.0 \\
-5670.87 & 23.0 & 1.08 & -2.703 & 0.0 & 0.0 & 0.0 \\
-5670.87 & 23.0 & 1.08 & -1.858 & 0.0 & 0.0 & 0.0 \\
-5670.87 & 23.0 & 1.08 & -1.589 & 0.0 & 0.0 & 0.0 \\
-5670.875 & 23.0 & 1.08 & -2.858 & 0.0 & 0.0 & 0.0 \\
-5670.875 & 23.0 & 1.08 & -1.963 & 0.0 & 0.0 & 0.0 \\
-5670.875 & 23.0 & 1.08 & -1.759 & 0.0 & 0.0 & 0.0 \\
-5670.878 & 23.0 & 1.08 & -2.159 & 0.0 & 0.0 & 0.0 \\
-5670.878 & 23.0 & 1.08 & -1.963 & 0.0 & 0.0 & 0.0 \\
-5670.88 & 23.0 & 1.08 & -2.226 & 0.0 & 0.0 & 0.0 \\
5703.5552 & 23.0 & 1.0509 & -0.779 & 89.7 & 82.4 & 29.4 \\
-5703.5688 & 23.0 & 1.0509 & -0.995 & 0.0 & 0.0 & 0.0 \\
-5703.5688 & 23.0 & 1.0509 & -1.405 & 0.0 & 0.0 & 0.0 \\
-5703.5796 & 23.0 & 1.0509 & -1.244 & 0.0 & 0.0 & 0.0 \\
-5703.5796 & 23.0 & 1.0509 & -1.278 & 0.0 & 0.0 & 0.0 \\
-5703.5811 & 23.0 & 1.0509 & -2.27 & 0.0 & 0.0 & 0.0 \\
-5703.5889 & 23.0 & 1.0509 & -1.717 & 0.0 & 0.0 & 0.0 \\
-5703.5889 & 23.0 & 1.0509 & -1.252 & 0.0 & 0.0 & 0.0 \\
-5703.5898 & 23.0 & 1.0509 & -1.842 & 0.0 & 0.0 & 0.0 \\
-5703.5962 & 23.0 & 1.0509 & -1.592 & 0.0 & 0.0 & 0.0 \\
-5703.5962 & 23.0 & 1.0509 & -1.416 & 0.0 & 0.0 & 0.0 \\
-5703.6011 & 23.0 & 1.0509 & -1.416 & 0.0 & 0.0 & 0.0 \\
5727.027 & 23.0 & 1.081 & -2.993 & 108.7 & 99.8 & 40.0 \\
-5727.027 & 23.0 & 1.081 & -1.692 & 0.0 & 0.0 & 0.0 \\
-5727.027 & 23.0 & 1.081 & -0.684 & 0.0 & 0.0 & 0.0 \\
-5727.039 & 23.0 & 1.081 & -2.595 & 0.0 & 0.0 & 0.0 \\
-5727.039 & 23.0 & 1.081 & -1.481 & 0.0 & 0.0 & 0.0 \\
-5727.039 & 23.0 & 1.081 & -0.789 & 0.0 & 0.0 & 0.0 \\
-5727.049 & 23.0 & 1.081 & -2.391 & 0.0 & 0.0 & 0.0 \\
-5727.049 & 23.0 & 1.081 & -1.408 & 0.0 & 0.0 & 0.0 \\
-5727.049 & 23.0 & 1.081 & -0.905 & 0.0 & 0.0 & 0.0 \\
-5727.058 & 23.0 & 1.081 & -2.294 & 0.0 & 0.0 & 0.0 \\
-5727.058 & 23.0 & 1.081 & -1.402 & 0.0 & 0.0 & 0.0 \\
-5727.058 & 23.0 & 1.081 & -1.034 & 0.0 & 0.0 & 0.0 \\
-5727.065 & 23.0 & 1.081 & -2.294 & 0.0 & 0.0 & 0.0 \\
-5727.065 & 23.0 & 1.081 & -1.449 & 0.0 & 0.0 & 0.0 \\
-5727.065 & 23.0 & 1.081 & -1.18 & 0.0 & 0.0 & 0.0 \\
-5727.07 & 23.0 & 1.081 & -2.449 & 0.0 & 0.0 & 0.0 \\
-5727.07 & 23.0 & 1.081 & -1.554 & 0.0 & 0.0 & 0.0 \\
-5727.07 & 23.0 & 1.081 & -1.35 & 0.0 & 0.0 & 0.0 \\
-5727.074 & 23.0 & 1.081 & -1.75 & 0.0 & 0.0 & 0.0 \\
-5727.074 & 23.0 & 1.081 & -1.554 & 0.0 & 0.0 & 0.0 \\
-5727.076 & 23.0 & 1.081 & -1.817 & 0.0 & 0.0 & 0.0 \\
5727.6191 & 23.0 & 1.0509 & -1.892 & 54.9 & 44.3 & 9.4 \\
-5727.6191 & 23.0 & 1.0509 & -1.481 & 0.0 & 0.0 & 0.0 \\
-5727.6533 & 23.0 & 1.0509 & -2.097 & 0.0 & 0.0 & 0.0 \\
-5727.6533 & 23.0 & 1.0509 & -1.778 & 0.0 & 0.0 & 0.0 \\
-5727.6538 & 23.0 & 1.0509 & -1.892 & 0.0 & 0.0 & 0.0 \\
-5727.6812 & 23.0 & 1.0509 & -1.903 & 0.0 & 0.0 & 0.0 \\
-5727.6812 & 23.0 & 1.0509 & -1.778 & 0.0 & 0.0 & 0.0 \\
-5727.7007 & 23.0 & 1.0509 & -2.079 & 0.0 & 0.0 & 0.0 \\
-5727.7021 & 23.0 & 1.0509 & -1.903 & 0.0 & 0.0 & 0.0 \\
5737.0269 & 23.0 & 1.0636 & -1.382 & 61.7 & 50.3 & 10.8 \\
-5737.0366 & 23.0 & 1.0636 & -2.081 & 0.0 & 0.0 & 0.0 \\
-5737.041 & 23.0 & 1.0636 & -2.081 & 0.0 & 0.0 & 0.0 \\
-5737.0508 & 23.0 & 1.0636 & -1.674 & 0.0 & 0.0 & 0.0 \\
-5737.0586 & 23.0 & 1.0636 & -1.9 & 0.0 & 0.0 & 0.0 \\
-5737.063 & 23.0 & 1.0636 & -1.9 & 0.0 & 0.0 & 0.0 \\
-5737.0708 & 23.0 & 1.0636 & -2.08 & 0.0 & 0.0 & 0.0 \\
-5737.0771 & 23.0 & 1.0636 & -1.869 & 0.0 & 0.0 & 0.0 \\
-5737.0801 & 23.0 & 1.0636 & -1.869 & 0.0 & 0.0 & 0.0 \\
-5737.0859 & 23.0 & 1.0636 & -2.797 & 0.0 & 0.0 & 0.0 \\
-5737.0908 & 23.0 & 1.0636 & -1.933 & 0.0 & 0.0 & 0.0 \\
-5737.0928 & 23.0 & 1.0636 & -1.933 & 0.0 & 0.0 & 0.0 \\
-5737.0977 & 23.0 & 1.0636 & -4.04 & 0.0 & 0.0 & 0.0 \\
-5737.1006 & 23.0 & 1.0636 & -2.132 & 0.0 & 0.0 & 0.0 \\
-5737.1035 & 23.0 & 1.0636 & -2.132 & 0.0 & 0.0 & 0.0 \\
-5737.1055 & 23.0 & 1.0636 & -2.387 & 0.0 & 0.0 & 0.0 \\
6039.727 & 23.0 & 1.063 & -1.854 & 51.6 & 44.2 & 12.1 \\
-6039.729 & 23.0 & 1.063 & -1.854 & 0.0 & 0.0 & 0.0 \\
-6039.73 & 23.0 & 1.063 & -2.03 & 0.0 & 0.0 & 0.0 \\
-6039.733 & 23.0 & 1.063 & -1.69 & 0.0 & 0.0 & 0.0 \\
-6039.733 & 23.0 & 1.063 & -2.155 & 0.0 & 0.0 & 0.0 \\
-6039.734 & 23.0 & 1.063 & -2.28 & 0.0 & 0.0 & 0.0 \\
-6039.738 & 23.0 & 1.063 & -1.682 & 0.0 & 0.0 & 0.0 \\
-6039.738 & 23.0 & 1.063 & -1.716 & 0.0 & 0.0 & 0.0 \\
-6039.739 & 23.0 & 1.063 & -2.708 & 0.0 & 0.0 & 0.0 \\
-6039.744 & 23.0 & 1.063 & -1.843 & 0.0 & 0.0 & 0.0 \\
-6039.744 & 23.0 & 1.063 & -1.433 & 0.0 & 0.0 & 0.0 \\
-6039.751 & 23.0 & 1.063 & -1.217 & 0.0 & 0.0 & 0.0 \\
6081.417 & 23.0 & 1.051 & -1.66 & 64.3 & 55.1 & 14.5 \\
-6081.417 & 23.0 & 1.051 & -1.484 & 0.0 & 0.0 & 0.0 \\
-6081.427 & 23.0 & 1.051 & -1.484 & 0.0 & 0.0 & 0.0 \\
-6081.428 & 23.0 & 1.051 & -1.359 & 0.0 & 0.0 & 0.0 \\
-6081.442 & 23.0 & 1.051 & -1.359 & 0.0 & 0.0 & 0.0 \\
-6081.442 & 23.0 & 1.051 & -1.677 & 0.0 & 0.0 & 0.0 \\
-6081.442 & 23.0 & 1.051 & -1.472 & 0.0 & 0.0 & 0.0 \\
-6081.46 & 23.0 & 1.051 & -1.472 & 0.0 & 0.0 & 0.0 \\
6090.199 & 23.0 & 1.08 & -0.692 & 85.8 & 79.5 & 34.2 \\
-6090.207 & 23.0 & 1.08 & -0.833 & 0.0 & 0.0 & 0.0 \\
-6090.213 & 23.0 & 1.08 & -0.997 & 0.0 & 0.0 & 0.0 \\
-6090.213 & 23.0 & 1.08 & -1.532 & 0.0 & 0.0 & 0.0 \\
-6090.218 & 23.0 & 1.08 & -1.195 & 0.0 & 0.0 & 0.0 \\
-6090.218 & 23.0 & 1.08 & -1.336 & 0.0 & 0.0 & 0.0 \\
-6090.223 & 23.0 & 1.08 & -1.45 & 0.0 & 0.0 & 0.0 \\
-6090.223 & 23.0 & 1.08 & -1.282 & 0.0 & 0.0 & 0.0 \\
-6090.225 & 23.0 & 1.08 & -2.646 & 0.0 & 0.0 & 0.0 \\
-6090.226 & 23.0 & 1.08 & -1.304 & 0.0 & 0.0 & 0.0 \\
-6090.227 & 23.0 & 1.08 & -1.838 & 0.0 & 0.0 & 0.0 \\
-6090.228 & 23.0 & 1.08 & -2.236 & 0.0 & 0.0 & 0.0 \\
-6090.229 & 23.0 & 1.08 & -1.394 & 0.0 & 0.0 & 0.0 \\
-6090.231 & 23.0 & 1.08 & -1.583 & 0.0 & 0.0 & 0.0 \\
-6090.231 & 23.0 & 1.08 & -2.014 & 0.0 & 0.0 & 0.0 \\
-6090.232 & 23.0 & 1.08 & -1.889 & 0.0 & 0.0 & 0.0 \\
-6090.233 & 23.0 & 1.08 & -1.868 & 0.0 & 0.0 & 0.0 \\
-6090.233 & 23.0 & 1.08 & -1.838 & 0.0 & 0.0 & 0.0 \\
6111.6501 & 23.0 & 1.043 & -0.714 & 65.5 & 54.0 & 11.7 \\
6119.51 & 23.0 & 1.064 & -1.825 & 72.0 & 65.3 & 21.9 \\
-6119.514 & 23.0 & 1.064 & -1.386 & 0.0 & 0.0 & 0.0 \\
-6119.516 & 23.0 & 1.064 & -1.524 & 0.0 & 0.0 & 0.0 \\
-6119.519 & 23.0 & 1.064 & -1.524 & 0.0 & 0.0 & 0.0 \\
-6119.519 & 23.0 & 1.064 & -1.103 & 0.0 & 0.0 & 0.0 \\
-6119.521 & 23.0 & 1.064 & -1.36 & 0.0 & 0.0 & 0.0 \\
-6119.527 & 23.0 & 1.064 & -1.7 & 0.0 & 0.0 & 0.0 \\
-6119.527 & 23.0 & 1.064 & -0.887 & 0.0 & 0.0 & 0.0 \\
-6119.528 & 23.0 & 1.064 & -1.352 & 0.0 & 0.0 & 0.0 \\
-6119.535 & 23.0 & 1.064 & -1.95 & 0.0 & 0.0 & 0.0 \\
-6119.537 & 23.0 & 1.064 & -1.513 & 0.0 & 0.0 & 0.0 \\
-6119.546 & 23.0 & 1.064 & -2.378 & 0.0 & 0.0 & 0.0 \\
6135.3418 & 23.0 & 1.0509 & -1.552 & 54.3 & 43.4 & 10.2 \\
-6135.3418 & 23.0 & 1.0509 & -1.531 & 0.0 & 0.0 & 0.0 \\
-6135.3428 & 23.0 & 1.0509 & -1.677 & 0.0 & 0.0 & 0.0 \\
-6135.3818 & 23.0 & 1.0509 & -2.008 & 0.0 & 0.0 & 0.0 \\
-6135.3818 & 23.0 & 1.0509 & -1.531 & 0.0 & 0.0 & 0.0 \\
-6135.3833 & 23.0 & 1.0509 & -1.21 & 0.0 & 0.0 & 0.0 \\
6216.3252 & 23.0 & 0.2753 & -1.46 & 101.6 & 89.1 & 35.8 \\
-6216.3428 & 23.0 & 0.2753 & -1.601 & 0.0 & 0.0 & 0.0 \\
-6216.3579 & 23.0 & 0.2753 & -1.765 & 0.0 & 0.0 & 0.0 \\
-6216.3721 & 23.0 & 0.2753 & -2.3 & 0.0 & 0.0 & 0.0 \\
-6216.3721 & 23.0 & 0.2753 & -1.963 & 0.0 & 0.0 & 0.0 \\
-6216.3828 & 23.0 & 0.2753 & -2.104 & 0.0 & 0.0 & 0.0 \\
-6216.3843 & 23.0 & 0.2753 & -2.218 & 0.0 & 0.0 & 0.0 \\
-6216.3921 & 23.0 & 0.2753 & -2.05 & 0.0 & 0.0 & 0.0 \\
-6216.3955 & 23.0 & 0.2753 & -2.606 & 0.0 & 0.0 & 0.0 \\
-6216.3989 & 23.0 & 0.2753 & -2.072 & 0.0 & 0.0 & 0.0 \\
-6216.4038 & 23.0 & 0.2753 & -2.163 & 0.0 & 0.0 & 0.0 \\
-6216.4082 & 23.0 & 0.2753 & -2.351 & 0.0 & 0.0 & 0.0 \\
-6216.4111 & 23.0 & 0.2753 & -3.414 & 0.0 & 0.0 & 0.0 \\
-6216.415 & 23.0 & 0.2753 & -2.636 & 0.0 & 0.0 & 0.0 \\
-6216.416 & 23.0 & 0.2753 & -3.004 & 0.0 & 0.0 & 0.0 \\
-6216.418 & 23.0 & 0.2753 & -2.606 & 0.0 & 0.0 & 0.0 \\
-6216.418 & 23.0 & 0.2753 & -2.782 & 0.0 & 0.0 & 0.0 \\
-6216.4189 & 23.0 & 0.2753 & -2.657 & 0.0 & 0.0 & 0.0 \\
6224.4609 & 23.0 & 0.2866 & -3.519 & 43.5 & 33.4 & 6.0 \\
-6224.4707 & 23.0 & 0.2866 & -3.315 & 0.0 & 0.0 & 0.0 \\
-6224.48 & 23.0 & 0.2866 & -3.25 & 0.0 & 0.0 & 0.0 \\
-6224.4893 & 23.0 & 0.2866 & -3.257 & 0.0 & 0.0 & 0.0 \\
-6224.4961 & 23.0 & 0.2866 & -2.616 & 0.0 & 0.0 & 0.0 \\
-6224.4961 & 23.0 & 0.2866 & -3.323 & 0.0 & 0.0 & 0.0 \\
-6224.501 & 23.0 & 0.2866 & -2.803 & 0.0 & 0.0 & 0.0 \\
-6224.5029 & 23.0 & 0.2866 & -3.461 & 0.0 & 0.0 & 0.0 \\
-6224.5049 & 23.0 & 0.2866 & -3.022 & 0.0 & 0.0 & 0.0 \\
-6224.5078 & 23.0 & 0.2866 & -3.285 & 0.0 & 0.0 & 0.0 \\
-6224.5098 & 23.0 & 0.2866 & -3.741 & 0.0 & 0.0 & 0.0 \\
-6224.5112 & 23.0 & 0.2866 & -3.616 & 0.0 & 0.0 & 0.0 \\
-6224.5127 & 23.0 & 0.2866 & -4.063 & 0.0 & 0.0 & 0.0 \\
-6224.5146 & 23.0 & 0.2866 & -4.762 & 0.0 & 0.0 & 0.0 \\
-6224.5205 & 23.0 & 0.2866 & -3.741 & 0.0 & 0.0 & 0.0 \\
-6224.5239 & 23.0 & 0.2866 & -3.461 & 0.0 & 0.0 & 0.0 \\
-6224.5283 & 23.0 & 0.2866 & -3.323 & 0.0 & 0.0 & 0.0 \\
-6224.5312 & 23.0 & 0.2866 & -3.257 & 0.0 & 0.0 & 0.0 \\
-6224.5332 & 23.0 & 0.2866 & -3.25 & 0.0 & 0.0 & 0.0 \\
-6224.5342 & 23.0 & 0.2866 & -3.315 & 0.0 & 0.0 & 0.0 \\
-6224.5352 & 23.0 & 0.2866 & -3.519 & 0.0 & 0.0 & 0.0 \\
6242.7979 & 23.0 & 0.2619 & -2.017 & 64.8 & 52.9 & 20.9 \\
-6242.7979 & 23.0 & 0.2619 & -2.484 & 0.0 & 0.0 & 0.0 \\
-6242.8291 & 23.0 & 0.2619 & -2.338 & 0.0 & 0.0 & 0.0 \\
-6242.8369 & 23.0 & 0.2619 & -2.338 & 0.0 & 0.0 & 0.0 \\
-6242.8521 & 23.0 & 0.2619 & -2.359 & 0.0 & 0.0 & 0.0 \\
-6242.8682 & 23.0 & 0.2619 & -2.815 & 0.0 & 0.0 & 0.0 \\
6243.0449 & 23.0 & 0.3006 & -2.751 & 102.5 & 90.9 & 27.5 \\
-6243.061 & 23.0 & 0.3006 & -2.536 & 0.0 & 0.0 & 0.0 \\
-6243.0752 & 23.0 & 0.3006 & -2.459 & 0.0 & 0.0 & 0.0 \\
-6243.0869 & 23.0 & 0.3006 & -2.448 & 0.0 & 0.0 & 0.0 \\
-6243.0879 & 23.0 & 0.3006 & -1.688 & 0.0 & 0.0 & 0.0 \\
-6243.0981 & 23.0 & 0.3006 & -1.824 & 0.0 & 0.0 & 0.0 \\
-6243.0986 & 23.0 & 0.3006 & -2.491 & 0.0 & 0.0 & 0.0 \\
-6243.106 & 23.0 & 0.3006 & -1.972 & 0.0 & 0.0 & 0.0 \\
-6243.1094 & 23.0 & 0.3006 & -2.594 & 0.0 & 0.0 & 0.0 \\
-6243.1143 & 23.0 & 0.3006 & -2.131 & 0.0 & 0.0 & 0.0 \\
-6243.1191 & 23.0 & 0.3006 & -2.815 & 0.0 & 0.0 & 0.0 \\
-6243.1201 & 23.0 & 0.3006 & -2.3 & 0.0 & 0.0 & 0.0 \\
-6243.125 & 23.0 & 0.3006 & -2.467 & 0.0 & 0.0 & 0.0 \\
-6243.1294 & 23.0 & 0.3006 & -2.605 & 0.0 & 0.0 & 0.0 \\
-6243.1318 & 23.0 & 0.3006 & -2.619 & 0.0 & 0.0 & 0.0 \\
-6243.1401 & 23.0 & 0.3006 & -2.751 & 0.0 & 0.0 & 0.0 \\
-6243.1421 & 23.0 & 0.3006 & -2.815 & 0.0 & 0.0 & 0.0 \\
-6243.1426 & 23.0 & 0.3006 & -2.536 & 0.0 & 0.0 & 0.0 \\
-6243.145 & 23.0 & 0.3006 & -2.594 & 0.0 & 0.0 & 0.0 \\
-6243.1455 & 23.0 & 0.3006 & -2.491 & 0.0 & 0.0 & 0.0 \\
-6243.1455 & 23.0 & 0.3006 & -2.459 & 0.0 & 0.0 & 0.0 \\
-6243.147 & 23.0 & 0.3006 & -2.448 & 0.0 & 0.0 & 0.0 \\
6251.771 & 23.0 & 0.286 & -2.924 & 80.5 & 67.4 & 16.0 \\
-6251.788 & 23.0 & 0.286 & -2.72 & 0.0 & 0.0 & 0.0 \\
-6251.804 & 23.0 & 0.286 & -2.655 & 0.0 & 0.0 & 0.0 \\
-6251.806 & 23.0 & 0.286 & -2.021 & 0.0 & 0.0 & 0.0 \\
-6251.817 & 23.0 & 0.286 & -2.662 & 0.0 & 0.0 & 0.0 \\
-6251.818 & 23.0 & 0.286 & -2.208 & 0.0 & 0.0 & 0.0 \\
-6251.829 & 23.0 & 0.286 & -2.728 & 0.0 & 0.0 & 0.0 \\
-6251.829 & 23.0 & 0.286 & -2.427 & 0.0 & 0.0 & 0.0 \\
-6251.837 & 23.0 & 0.286 & -2.69 & 0.0 & 0.0 & 0.0 \\
-6251.839 & 23.0 & 0.286 & -2.866 & 0.0 & 0.0 & 0.0 \\
-6251.844 & 23.0 & 0.286 & -3.021 & 0.0 & 0.0 & 0.0 \\
-6251.848 & 23.0 & 0.286 & -3.146 & 0.0 & 0.0 & 0.0 \\
-6251.849 & 23.0 & 0.286 & -3.468 & 0.0 & 0.0 & 0.0 \\
-6251.853 & 23.0 & 0.286 & -4.167 & 0.0 & 0.0 & 0.0 \\
-6251.853 & 23.0 & 0.286 & -2.924 & 0.0 & 0.0 & 0.0 \\
-6251.859 & 23.0 & 0.286 & -3.146 & 0.0 & 0.0 & 0.0 \\
-6251.859 & 23.0 & 0.286 & -2.72 & 0.0 & 0.0 & 0.0 \\
-6251.862 & 23.0 & 0.286 & -2.655 & 0.0 & 0.0 & 0.0 \\
-6251.863 & 23.0 & 0.286 & -2.866 & 0.0 & 0.0 & 0.0 \\
-6251.864 & 23.0 & 0.286 & -2.728 & 0.0 & 0.0 & 0.0 \\
-6251.864 & 23.0 & 0.286 & -2.662 & 0.0 & 0.0 & 0.0 \\
6274.607 & 23.0 & 0.267 & -2.932 & 53.1 & 44.8 & 8.8 \\
-6274.629 & 23.0 & 0.267 & -2.455 & 0.0 & 0.0 & 0.0 \\
-6274.641 & 23.0 & 0.267 & -2.476 & 0.0 & 0.0 & 0.0 \\
-6274.655 & 23.0 & 0.267 & -2.134 & 0.0 & 0.0 & 0.0 \\
-6274.657 & 23.0 & 0.267 & -2.455 & 0.0 & 0.0 & 0.0 \\
-6274.678 & 23.0 & 0.267 & -2.601 & 0.0 & 0.0 & 0.0 \\
6285.098 & 23.0 & 0.275 & -3.568 & 59.3 & 48.6 & 10.2 \\
-6285.117 & 23.0 & 0.275 & -3.14 & 0.0 & 0.0 & 0.0 \\
-6285.122 & 23.0 & 0.275 & -2.703 & 0.0 & 0.0 & 0.0 \\
-6285.134 & 23.0 & 0.275 & -2.89 & 0.0 & 0.0 & 0.0 \\
-6285.137 & 23.0 & 0.275 & -2.542 & 0.0 & 0.0 & 0.0 \\
-6285.148 & 23.0 & 0.275 & -2.714 & 0.0 & 0.0 & 0.0 \\
-6285.149 & 23.0 & 0.275 & -2.55 & 0.0 & 0.0 & 0.0 \\
-6285.152 & 23.0 & 0.275 & -2.077 & 0.0 & 0.0 & 0.0 \\
-6285.157 & 23.0 & 0.275 & -2.714 & 0.0 & 0.0 & 0.0 \\
-6285.162 & 23.0 & 0.275 & -2.293 & 0.0 & 0.0 & 0.0 \\
-6285.168 & 23.0 & 0.275 & -2.576 & 0.0 & 0.0 & 0.0 \\
-6285.172 & 23.0 & 0.275 & -3.015 & 0.0 & 0.0 & 0.0 \\
6292.7583 & 23.0 & 0.2866 & -4.055 & 61.4 & 51.9 & 13.3 \\
-6292.7759 & 23.0 & 0.2866 & -3.645 & 0.0 & 0.0 & 0.0 \\
-6292.7886 & 23.0 & 0.2866 & -2.941 & 0.0 & 0.0 & 0.0 \\
-6292.791 & 23.0 & 0.2866 & -3.423 & 0.0 & 0.0 & 0.0 \\
-6292.8008 & 23.0 & 0.2866 & -2.745 & 0.0 & 0.0 & 0.0 \\
-6292.8037 & 23.0 & 0.2866 & -3.298 & 0.0 & 0.0 & 0.0 \\
-6292.8115 & 23.0 & 0.2866 & -2.691 & 0.0 & 0.0 & 0.0 \\
-6292.8164 & 23.0 & 0.2866 & -3.247 & 0.0 & 0.0 & 0.0 \\
-6292.8193 & 23.0 & 0.2866 & -2.713 & 0.0 & 0.0 & 0.0 \\
-6292.8242 & 23.0 & 0.2866 & -2.101 & 0.0 & 0.0 & 0.0 \\
-6292.8247 & 23.0 & 0.2866 & -3.277 & 0.0 & 0.0 & 0.0 \\
-6292.8262 & 23.0 & 0.2866 & -2.804 & 0.0 & 0.0 & 0.0 \\
-6292.8301 & 23.0 & 0.2866 & -2.992 & 0.0 & 0.0 & 0.0 \\
-6292.8311 & 23.0 & 0.2866 & -2.242 & 0.0 & 0.0 & 0.0 \\
-6292.8369 & 23.0 & 0.2866 & -2.406 & 0.0 & 0.0 & 0.0 \\
-6292.8398 & 23.0 & 0.2866 & -3.247 & 0.0 & 0.0 & 0.0 \\
-6292.8398 & 23.0 & 0.2866 & -2.604 & 0.0 & 0.0 & 0.0 \\
-6292.8413 & 23.0 & 0.2866 & -2.859 & 0.0 & 0.0 & 0.0 \\
6531.3877 & 23.0 & 1.2181 & -2.487 & 38.6 & 29.5 & 6.5 \\
-6531.3911 & 23.0 & 1.2181 & -2.232 & 0.0 & 0.0 & 0.0 \\
-6531.3911 & 23.0 & 1.2181 & -2.232 & 0.0 & 0.0 & 0.0 \\
-6531.394 & 23.0 & 1.2181 & -4.14 & 0.0 & 0.0 & 0.0 \\
-6531.3975 & 23.0 & 1.2181 & -2.033 & 0.0 & 0.0 & 0.0 \\
-6531.3989 & 23.0 & 1.2181 & -2.033 & 0.0 & 0.0 & 0.0 \\
-6531.4033 & 23.0 & 1.2181 & -2.897 & 0.0 & 0.0 & 0.0 \\
-6531.4082 & 23.0 & 1.2181 & -1.969 & 0.0 & 0.0 & 0.0 \\
-6531.4092 & 23.0 & 1.2181 & -1.969 & 0.0 & 0.0 & 0.0 \\
-6531.4141 & 23.0 & 1.2181 & -2.18 & 0.0 & 0.0 & 0.0 \\
-6531.4209 & 23.0 & 1.2181 & -2.0 & 0.0 & 0.0 & 0.0 \\
-6531.4219 & 23.0 & 1.2181 & -2.0 & 0.0 & 0.0 & 0.0 \\
-6531.4287 & 23.0 & 1.2181 & -1.774 & 0.0 & 0.0 & 0.0 \\
-6531.436 & 23.0 & 1.2181 & -2.181 & 0.0 & 0.0 & 0.0 \\
-6531.438 & 23.0 & 1.2181 & -2.181 & 0.0 & 0.0 & 0.0 \\
-6531.4458 & 23.0 & 1.2181 & -1.482 & 0.0 & 0.0 & 0.0 \\
4511.9 & 24.0 & 3.09 & -0.39 & 69.2 & 65.2 & 40.3 \\
4535.1268 & 24.0 & 2.544 & -0.993 & 60.6 & 57.3 & 30.8 \\
4541.0601 & 24.0 & 2.545 & -1.143 & 52.3 & 50.3 & 24.9 \\
4575.11 & 24.0 & 3.37 & -1.004 & 32.6 & 28.0 & 9.0 \\
4600.75 & 24.0 & 1.0 & -1.457 & 112.3 & 106.6 & 82.1 \\
4626.18 & 24.0 & 0.97 & -1.467 & 106.4 & 101.9 & 78.9 \\
4633.259 & 24.0 & 3.125 & -1.11 & 35.5 & 32.9 & 10.1 \\
4700.5988 & 24.0 & 2.71 & -1.255 & 39.5 & 36.9 & 13.9 \\
4708.0174 & 24.0 & 3.168 & 0.09 & 82.3 & 78.0 & 55.5 \\
4730.72 & 24.0 & 3.08 & -0.345 & 79.2 & 76.8 & 47.3 \\
4745.2702 & 24.0 & 2.708 & -1.38 & 42.7 & 39.9 & 15.5 \\
4767.86 & 24.0 & 3.56 & -0.599 & 42.3 & 38.4 & 16.8 \\
4775.14 & 24.0 & 3.55 & -1.025 & 29.1 & 28.7 & 7.3 \\
4789.3401 & 24.0 & 2.544 & -0.348 & 93.7 & 90.7 & 62.4 \\
4801.0477 & 24.0 & 3.122 & -0.131 & 74.0 & 71.2 & 47.4 \\
4885.7334 & 24.0 & 2.544 & -1.055 & 60.1 & 55.3 & 30.5 \\
4936.3355 & 24.0 & 3.113 & -0.237 & 76.7 & 72.8 & 44.2 \\
4953.7144 & 24.0 & 3.122 & -1.48 & 24.4 & 19.5 & 5.6 \\
4964.93 & 24.0 & 0.94 & -2.577 & 77.6 & 73.2 & 39.4 \\
5214.14 & 24.0 & 3.37 & -0.784 & 43.6 & 40.1 & 17.6 \\
5238.96 & 24.0 & 2.71 & -1.43 & 47.1 & 43.1 & 16.4 \\
5241.454 & 24.0 & 2.71 & -1.92 & 19.9 & 15.8 & 4.2 \\
5247.57 & 24.0 & 0.96 & -1.618 & 119.8 & 114.6 & 79.1 \\
5272.0079 & 24.0 & 3.449 & -0.421 & 54.1 & 51.3 & 23.6 \\
5287.2011 & 24.0 & 3.438 & -0.888 & 35.5 & 31.7 & 11.4 \\
5296.691 & 24.0 & 0.983 & -1.41 & 144.3 & 137.6 & 92.4 \\
5297.39 & 24.0 & 2.9 & 0.0 & 117.8 & 111.1 & 79.8 \\
5300.7429 & 24.0 & 0.983 & -2.083 & 102.2 & 94.8 & 59.1 \\
5304.184 & 24.0 & 3.464 & -0.681 & 44.6 & 39.9 & 15.1 \\
5480.51 & 24.0 & 3.5 & -0.92 & 31.3 & 26.6 & 10.1 \\
5574.39 & 24.0 & 4.45 & -0.72 & 11.3 & 10.9 & 5.2 \\
5628.6214 & 24.0 & 3.422 & -0.756 & 43.3 & 38.9 & 15.1 \\
5719.8089 & 24.0 & 3.013 & -1.62 & 22.1 & 19.1 & 8.0 \\
5781.1632 & 24.0 & 3.011 & -1.0 & 48.8 & 42.6 & 16.0 \\
5783.073 & 24.0 & 3.232 & -0.48 & 67.7 & 61.8 & 31.4 \\
5783.87 & 24.0 & 3.322 & -0.29 & 88.4 & 83.3 & 43.9 \\
5785.0243 & 24.0 & 3.321 & -0.38 & 74.7 & 68.7 & 34.1 \\
5787.93 & 24.0 & 3.322 & -0.08 & 83.7 & 79.8 & 46.8 \\
5844.5919 & 24.0 & 3.013 & -1.77 & 23.6 & 19.5 & 5.2 \\
6330.1 & 24.0 & 0.941 & -2.9 & 72.7 & 68.3 & 27.9 \\
6882.4772 & 24.0 & 3.438 & -0.375 & 179.3 & 171.5 & 34.2 \\
6882.997 & 24.0 & 3.438 & -0.42 & 73.0 & 67.1 & 29.9 \\
4588.1997 & 24.1 & 4.071 & -0.594 & 68.8 & 70.3 & 68.0 \\
4592.05 & 24.1 & 4.071 & -1.252 & 54.3 & 53.1 & 46.0 \\
4848.2365 & 24.1 & 3.864 & -1.16 & 71.5 & 69.8 & 60.2 \\
4884.61 & 24.1 & 3.86 & -2.069 & 37.3 & 35.4 & 25.6 \\
5237.328 & 24.1 & 4.073 & -1.087 & 57.0 & 57.5 & 50.4 \\
5246.7678 & 24.1 & 3.714 & -2.436 & 19.6 & 18.5 & 13.1 \\
5279.8769 & 24.1 & 4.073 & -1.909 & 17.6 & 17.2 & 16.2 \\
5305.87 & 24.1 & 3.827 & -1.97 & 30.6 & 29.6 & 24.7 \\
5308.42 & 24.1 & 4.07 & -1.79 & 39.9 & 37.4 & 25.9 \\
5310.686 & 24.1 & 4.072 & -2.144 & 15.9 & 15.1 & 12.6 \\
4502.2041 & 25.0 & 2.9197 & -0.61 & 93.6 & 90.4 & 58.3 \\
-4502.207 & 25.0 & 2.9197 & -1.528 & 0.0 & 0.0 & 0.0 \\
-4502.208 & 25.0 & 2.9197 & -2.745 & 0.0 & 0.0 & 0.0 \\
-4502.2109 & 25.0 & 2.9197 & -0.75 & 0.0 & 0.0 & 0.0 \\
-4502.2129 & 25.0 & 2.9197 & -2.393 & 0.0 & 0.0 & 0.0 \\
-4502.2129 & 25.0 & 2.9197 & -1.352 & 0.0 & 0.0 & 0.0 \\
-4502.2158 & 25.0 & 2.9197 & -0.908 & 0.0 & 0.0 & 0.0 \\
-4502.2173 & 25.0 & 2.9197 & -1.326 & 0.0 & 0.0 & 0.0 \\
-4502.2178 & 25.0 & 2.9197 & -2.268 & 0.0 & 0.0 & 0.0 \\
-4502.2197 & 25.0 & 2.9197 & -2.347 & 0.0 & 0.0 & 0.0 \\
-4502.2197 & 25.0 & 2.9197 & -1.393 & 0.0 & 0.0 & 0.0 \\
-4502.2197 & 25.0 & 2.9197 & -1.092 & 0.0 & 0.0 & 0.0 \\
-4502.2222 & 25.0 & 2.9197 & -1.569 & 0.0 & 0.0 & 0.0 \\
-4502.2222 & 25.0 & 2.9197 & -1.314 & 0.0 & 0.0 & 0.0 \\
-4502.2227 & 25.0 & 2.9197 & -1.599 & 0.0 & 0.0 & 0.0 \\
4709.693 & 25.0 & 2.8884 & -0.949 & 97.6 & 92.7 & 67.0 \\
-4709.698 & 25.0 & 2.8884 & -1.94 & 0.0 & 0.0 & 0.0 \\
-4709.701 & 25.0 & 2.8884 & -1.94 & 0.0 & 0.0 & 0.0 \\
-4709.706 & 25.0 & 2.8884 & -1.119 & 0.0 & 0.0 & 0.0 \\
-4709.711 & 25.0 & 2.8884 & -1.758 & 0.0 & 0.0 & 0.0 \\
-4709.713 & 25.0 & 2.8884 & -1.758 & 0.0 & 0.0 & 0.0 \\
-4709.717 & 25.0 & 2.8884 & -1.304 & 0.0 & 0.0 & 0.0 \\
-4709.721 & 25.0 & 2.8884 & -1.727 & 0.0 & 0.0 & 0.0 \\
-4709.723 & 25.0 & 2.8884 & -1.727 & 0.0 & 0.0 & 0.0 \\
-4709.726 & 25.0 & 2.8884 & -1.496 & 0.0 & 0.0 & 0.0 \\
-4709.729 & 25.0 & 2.8884 & -1.792 & 0.0 & 0.0 & 0.0 \\
-4709.73 & 25.0 & 2.8884 & -1.792 & 0.0 & 0.0 & 0.0 \\
-4709.733 & 25.0 & 2.8884 & -1.671 & 0.0 & 0.0 & 0.0 \\
-4709.735 & 25.0 & 2.8884 & -1.99 & 0.0 & 0.0 & 0.0 \\
-4709.736 & 25.0 & 2.8884 & -1.99 & 0.0 & 0.0 & 0.0 \\
-4709.737 & 25.0 & 2.8884 & -1.735 & 0.0 & 0.0 & 0.0 \\
4739.072 & 25.0 & 2.941 & -1.518 & 94.0 & 91.1 & 60.2 \\
-4739.072 & 25.0 & 2.941 & -1.041 & 0.0 & 0.0 & 0.0 \\
-4739.088 & 25.0 & 2.941 & -1.416 & 0.0 & 0.0 & 0.0 \\
-4739.088 & 25.0 & 2.941 & -1.59 & 0.0 & 0.0 & 0.0 \\
-4739.088 & 25.0 & 2.941 & -1.518 & 0.0 & 0.0 & 0.0 \\
-4739.1 & 25.0 & 2.941 & -1.416 & 0.0 & 0.0 & 0.0 \\
-4739.101 & 25.0 & 2.941 & -1.548 & 0.0 & 0.0 & 0.0 \\
-4739.101 & 25.0 & 2.941 & -3.125 & 0.0 & 0.0 & 0.0 \\
-4739.109 & 25.0 & 2.941 & -1.916 & 0.0 & 0.0 & 0.0 \\
-4739.109 & 25.0 & 2.941 & -1.548 & 0.0 & 0.0 & 0.0 \\
5004.887 & 25.0 & 2.92 & -4.332 & 44.5 & 39.7 & 14.0 \\
-5004.887 & 25.0 & 2.92 & -3.115 & 0.0 & 0.0 & 0.0 \\
-5004.887 & 25.0 & 2.92 & -2.197 & 0.0 & 0.0 & 0.0 \\
-5004.891 & 25.0 & 2.92 & -3.98 & 0.0 & 0.0 & 0.0 \\
-5004.891 & 25.0 & 2.92 & -2.939 & 0.0 & 0.0 & 0.0 \\
-5004.891 & 25.0 & 2.92 & -2.337 & 0.0 & 0.0 & 0.0 \\
-5004.894 & 25.0 & 2.92 & -3.855 & 0.0 & 0.0 & 0.0 \\
-5004.894 & 25.0 & 2.92 & -2.913 & 0.0 & 0.0 & 0.0 \\
-5004.894 & 25.0 & 2.92 & -2.495 & 0.0 & 0.0 & 0.0 \\
-5004.896 & 25.0 & 2.92 & -3.934 & 0.0 & 0.0 & 0.0 \\
-5004.896 & 25.0 & 2.92 & -2.98 & 0.0 & 0.0 & 0.0 \\
-5004.896 & 25.0 & 2.92 & -2.679 & 0.0 & 0.0 & 0.0 \\
-5004.898 & 25.0 & 2.92 & -3.186 & 0.0 & 0.0 & 0.0 \\
-5004.898 & 25.0 & 2.92 & -3.156 & 0.0 & 0.0 & 0.0 \\
-5004.898 & 25.0 & 2.92 & -2.901 & 0.0 & 0.0 & 0.0 \\
5255.2617 & 25.0 & 3.1325 & -4.07 & 97.6 & 94.3 & 43.4 \\
-5255.2666 & 25.0 & 3.1325 & -2.748 & 0.0 & 0.0 & 0.0 \\
-5255.2695 & 25.0 & 3.1325 & -1.949 & 0.0 & 0.0 & 0.0 \\
-5255.271 & 25.0 & 3.1325 & -3.911 & 0.0 & 0.0 & 0.0 \\
-5255.2773 & 25.0 & 3.1325 & -2.554 & 0.0 & 0.0 & 0.0 \\
-5255.2822 & 25.0 & 3.1325 & -1.855 & 0.0 & 0.0 & 0.0 \\
-5255.2822 & 25.0 & 3.1325 & -3.991 & 0.0 & 0.0 & 0.0 \\
-5255.2886 & 25.0 & 3.1325 & -2.502 & 0.0 & 0.0 & 0.0 \\
-5255.2949 & 25.0 & 3.1325 & -1.76 & 0.0 & 0.0 & 0.0 \\
-5255.2959 & 25.0 & 3.1325 & -4.313 & 0.0 & 0.0 & 0.0 \\
-5255.3052 & 25.0 & 3.1325 & -2.546 & 0.0 & 0.0 & 0.0 \\
-5255.312 & 25.0 & 3.1325 & -1.668 & 0.0 & 0.0 & 0.0 \\
-5255.3223 & 25.0 & 3.1325 & -2.739 & 0.0 & 0.0 & 0.0 \\
-5255.3311 & 25.0 & 3.1325 & -1.58 & 0.0 & 0.0 & 0.0 \\
-5255.3525 & 25.0 & 3.1325 & -1.497 & 0.0 & 0.0 & 0.0 \\
5394.6191 & 25.0 & 0.0 & -4.067 & 159.7 & 152.6 & 79.2 \\
-5394.6509 & 25.0 & 0.0 & -4.985 & 0.0 & 0.0 & 0.0 \\
-5394.6538 & 25.0 & 0.0 & -4.207 & 0.0 & 0.0 & 0.0 \\
-5394.6772 & 25.0 & 0.0 & -6.202 & 0.0 & 0.0 & 0.0 \\
-5394.6807 & 25.0 & 0.0 & -4.809 & 0.0 & 0.0 & 0.0 \\
-5394.6831 & 25.0 & 0.0 & -4.365 & 0.0 & 0.0 & 0.0 \\
-5394.7021 & 25.0 & 0.0 & -5.85 & 0.0 & 0.0 & 0.0 \\
-5394.7051 & 25.0 & 0.0 & -4.783 & 0.0 & 0.0 & 0.0 \\
-5394.707 & 25.0 & 0.0 & -4.549 & 0.0 & 0.0 & 0.0 \\
-5394.7212 & 25.0 & 0.0 & -5.725 & 0.0 & 0.0 & 0.0 \\
-5394.7227 & 25.0 & 0.0 & -4.85 & 0.0 & 0.0 & 0.0 \\
-5394.7246 & 25.0 & 0.0 & -4.771 & 0.0 & 0.0 & 0.0 \\
-5394.7339 & 25.0 & 0.0 & -5.804 & 0.0 & 0.0 & 0.0 \\
-5394.7358 & 25.0 & 0.0 & -5.056 & 0.0 & 0.0 & 0.0 \\
-5394.7358 & 25.0 & 0.0 & -5.026 & 0.0 & 0.0 & 0.0 \\
5399.45 & 25.0 & 3.85 & -1.162 & 95.6 & 88.8 & 37.6 \\
-5399.455 & 25.0 & 3.85 & -1.03 & 0.0 & 0.0 & 0.0 \\
-5399.465 & 25.0 & 3.85 & -1.53 & 0.0 & 0.0 & 0.0 \\
-5399.465 & 25.0 & 3.85 & -1.132 & 0.0 & 0.0 & 0.0 \\
-5399.478 & 25.0 & 3.85 & -2.74 & 0.0 & 0.0 & 0.0 \\
-5399.494 & 25.0 & 3.85 & -1.162 & 0.0 & 0.0 & 0.0 \\
-5399.497 & 25.0 & 3.85 & -1.204 & 0.0 & 0.0 & 0.0 \\
-5399.521 & 25.0 & 3.85 & -1.03 & 0.0 & 0.0 & 0.0 \\
-5399.522 & 25.0 & 3.85 & -0.655 & 0.0 & 0.0 & 0.0 \\
-5399.555 & 25.0 & 3.85 & -1.132 & 0.0 & 0.0 & 0.0 \\
5413.5933 & 25.0 & 3.859 & -1.81 & 66.3 & 63.1 & 20.9 \\
-5413.6279 & 25.0 & 3.859 & -1.379 & 0.0 & 0.0 & 0.0 \\
-5413.6377 & 25.0 & 3.859 & -1.266 & 0.0 & 0.0 & 0.0 \\
-5413.6577 & 25.0 & 3.859 & -1.266 & 0.0 & 0.0 & 0.0 \\
-5413.6968 & 25.0 & 3.859 & -0.902 & 0.0 & 0.0 & 0.0 \\
-5413.7017 & 25.0 & 3.859 & -1.363 & 0.0 & 0.0 & 0.0 \\
5420.252 & 25.0 & 2.1427 & -3.018 & 178.5 & 170.6 & 85.3 \\
-5420.2583 & 25.0 & 2.1427 & -2.988 & 0.0 & 0.0 & 0.0 \\
-5420.2666 & 25.0 & 2.1427 & -2.733 & 0.0 & 0.0 & 0.0 \\
-5420.2681 & 25.0 & 2.1427 & -3.766 & 0.0 & 0.0 & 0.0 \\
-5420.2773 & 25.0 & 2.1427 & -2.812 & 0.0 & 0.0 & 0.0 \\
-5420.291 & 25.0 & 2.1427 & -2.511 & 0.0 & 0.0 & 0.0 \\
-5420.2939 & 25.0 & 2.1427 & -3.687 & 0.0 & 0.0 & 0.0 \\
-5420.3071 & 25.0 & 2.1427 & -2.745 & 0.0 & 0.0 & 0.0 \\
-5420.3247 & 25.0 & 2.1427 & -2.327 & 0.0 & 0.0 & 0.0 \\
-5420.3291 & 25.0 & 2.1427 & -3.812 & 0.0 & 0.0 & 0.0 \\
-5420.3472 & 25.0 & 2.1427 & -2.771 & 0.0 & 0.0 & 0.0 \\
-5420.3701 & 25.0 & 2.1427 & -2.169 & 0.0 & 0.0 & 0.0 \\
-5420.376 & 25.0 & 2.1427 & -4.164 & 0.0 & 0.0 & 0.0 \\
-5420.3979 & 25.0 & 2.1427 & -2.947 & 0.0 & 0.0 & 0.0 \\
-5420.4248 & 25.0 & 2.1427 & -2.029 & 0.0 & 0.0 & 0.0 \\
6013.52 & 25.0 & 3.073 & -0.765 & 141.2 & 134.6 & 86.0 \\
-6013.545 & 25.0 & 3.073 & -0.977 & 0.0 & 0.0 & 0.0 \\
-6013.567 & 25.0 & 3.073 & -1.25 & 0.0 & 0.0 & 0.0 \\
-6013.573 & 25.0 & 3.073 & -1.454 & 0.0 & 0.0 & 0.0 \\
-6013.584 & 25.0 & 3.073 & -1.66 & 0.0 & 0.0 & 0.0 \\
-6013.587 & 25.0 & 3.073 & -1.308 & 0.0 & 0.0 & 0.0 \\
-6013.598 & 25.0 & 3.073 & -1.329 & 0.0 & 0.0 & 0.0 \\
-6013.605 & 25.0 & 3.073 & -1.484 & 0.0 & 0.0 & 0.0 \\
-6013.615 & 25.0 & 3.073 & -2.408 & 0.0 & 0.0 & 0.0 \\
-6013.615 & 25.0 & 3.073 & -1.806 & 0.0 & 0.0 & 0.0 \\
-6013.619 & 25.0 & 3.073 & -2.028 & 0.0 & 0.0 & 0.0 \\
-6013.619 & 25.0 & 3.073 & -1.852 & 0.0 & 0.0 & 0.0 \\
6016.613 & 25.0 & 3.073 & -1.444 & 144.4 & 140.6 & 93.8 \\
-6016.64 & 25.0 & 3.073 & -0.666 & 0.0 & 0.0 & 0.0 \\
-6016.64 & 25.0 & 3.073 & -1.281 & 0.0 & 0.0 & 0.0 \\
-6016.661 & 25.0 & 3.073 & -1.276 & 0.0 & 0.0 & 0.0 \\
-6016.662 & 25.0 & 3.073 & -0.929 & 0.0 & 0.0 & 0.0 \\
-6016.678 & 25.0 & 3.073 & -1.378 & 0.0 & 0.0 & 0.0 \\
-6016.679 & 25.0 & 3.073 & -1.26 & 0.0 & 0.0 & 0.0 \\
-6016.689 & 25.0 & 3.073 & -1.444 & 0.0 & 0.0 & 0.0 \\
-6016.69 & 25.0 & 3.073 & -1.707 & 0.0 & 0.0 & 0.0 \\
-6016.691 & 25.0 & 3.073 & -1.64 & 0.0 & 0.0 & 0.0 \\
-6016.697 & 25.0 & 3.073 & -2.406 & 0.0 & 0.0 & 0.0 \\
-6016.701 & 25.0 & 3.073 & -1.281 & 0.0 & 0.0 & 0.0 \\
-6016.707 & 25.0 & 3.073 & -1.64 & 0.0 & 0.0 & 0.0 \\
-6016.708 & 25.0 & 3.073 & -1.276 & 0.0 & 0.0 & 0.0 \\
-6016.709 & 25.0 & 3.073 & -1.378 & 0.0 & 0.0 & 0.0 \\
6021.746 & 25.0 & 3.075 & -2.668 & 151.8 & 144.8 & 94.0 \\
-6021.772 & 25.0 & 3.075 & -1.451 & 0.0 & 0.0 & 0.0 \\
-6021.774 & 25.0 & 3.075 & -2.316 & 0.0 & 0.0 & 0.0 \\
-6021.795 & 25.0 & 3.075 & -1.275 & 0.0 & 0.0 & 0.0 \\
-6021.798 & 25.0 & 3.075 & -2.191 & 0.0 & 0.0 & 0.0 \\
-6021.804 & 25.0 & 3.075 & -0.533 & 0.0 & 0.0 & 0.0 \\
-6021.813 & 25.0 & 3.075 & -1.249 & 0.0 & 0.0 & 0.0 \\
-6021.817 & 25.0 & 3.075 & -2.271 & 0.0 & 0.0 & 0.0 \\
-6021.821 & 25.0 & 3.075 & -0.673 & 0.0 & 0.0 & 0.0 \\
-6021.827 & 25.0 & 3.075 & -1.316 & 0.0 & 0.0 & 0.0 \\
-6021.834 & 25.0 & 3.075 & -0.831 & 0.0 & 0.0 & 0.0 \\
-6021.837 & 25.0 & 3.075 & -1.492 & 0.0 & 0.0 & 0.0 \\
-6021.843 & 25.0 & 3.075 & -1.015 & 0.0 & 0.0 & 0.0 \\
-6021.846 & 25.0 & 3.075 & -1.522 & 0.0 & 0.0 & 0.0 \\
-6021.847 & 25.0 & 3.075 & -1.237 & 0.0 & 0.0 & 0.0 \\
4365.896 & 26.0 & 2.99 & -2.25 & 68.4 & 67.0 & 50.0 \\
4389.245 & 26.0 & 0.052 & -4.583 & 99.4 & 95.3 & 70.9 \\
4445.471 & 26.0 & 0.087 & -5.441 & 76.7 & 72.2 & 40.3 \\
4602.001 & 26.0 & 1.608 & -3.154 & 100.3 & 95.6 & 71.1 \\
4630.12 & 26.0 & 2.28 & -2.52 & 103.0 & 97.3 & 72.4 \\
4635.85 & 26.0 & 2.85 & -2.34 & 75.4 & 72.1 & 54.0 \\
4683.56 & 26.0 & 2.83 & -2.41 & 83.3 & 80.3 & 53.8 \\
4690.14 & 26.0 & 3.69 & -1.61 & 85.8 & 83.6 & 58.7 \\
4749.95 & 26.0 & 4.56 & -1.24 & 60.4 & 57.8 & 35.9 \\
4779.439 & 26.0 & 3.415 & -2.02 & 61.9 & 60.3 & 39.2 \\
4779.44 & 26.0 & 3.42 & -2.16 & 61.9 & 60.3 & 39.2 \\
4788.76 & 26.0 & 3.24 & -1.73 & 90.8 & 88.3 & 66.4 \\
4799.41 & 26.0 & 3.64 & -2.13 & 56.9 & 54.9 & 34.2 \\
4802.88 & 26.0 & 3.64 & -1.514 & 81.4 & 79.3 & 60.1 \\
4808.15 & 26.0 & 3.25 & -2.69 & 53.0 & 49.5 & 26.3 \\
4950.1 & 26.0 & 3.42 & -1.56 & 102.6 & 99.5 & 72.0 \\
4961.91 & 26.0 & 3.63 & -2.19 & 56.7 & 52.3 & 26.4 \\
4994.129 & 26.0 & 0.915 & -3.08 & 147.6 & 137.8 & 104.7 \\
5016.48 & 26.0 & 4.26 & -1.373 & 58.7 & 54.9 & 33.0 \\
5044.211 & 26.0 & 2.851 & -2.058 & 108.5 & 103.1 & 72.5 \\
5054.64 & 26.0 & 3.64 & -1.98 & 69.8 & 67.8 & 39.4 \\
5109.65 & 26.0 & 4.3 & -0.73 & 110.0 & 104.6 & 74.6 \\
5127.679 & 26.0 & 0.052 & -6.125 & 53.9 & 49.7 & 18.3 \\
5141.74 & 26.0 & 2.42 & -2.23 & 126.9 & 122.2 & 82.5 \\
5197.94 & 26.0 & 4.3 & -1.54 & 61.9 & 59.1 & 36.0 \\
5198.71 & 26.0 & 2.22 & -2.14 & 144.4 & 136.2 & 95.3 \\
5223.18 & 26.0 & 3.64 & -1.783 & 54.8 & 51.9 & 28.0 \\
5225.525 & 26.0 & 0.11 & -4.789 & 109.6 & 104.3 & 72.3 \\
5228.38 & 26.0 & 4.22 & -1.19 & 80.4 & 77.3 & 56.0 \\
5242.49 & 26.0 & 3.63 & -0.99 & 113.5 & 109.6 & 84.4 \\
5243.77 & 26.0 & 4.26 & -0.99 & 91.0 & 86.4 & 61.7 \\
5247.05 & 26.0 & 0.087 & -4.961 & 100.6 & 95.6 & 64.5 \\
5250.208 & 26.0 & 0.121 & -4.938 & 100.7 & 96.5 & 65.4 \\
5253.02 & 26.0 & 2.28 & -3.84 & 47.6 & 42.8 & 17.9 \\
5285.13 & 26.0 & 4.43 & -1.54 & 50.0 & 47.6 & 26.3 \\
5288.52 & 26.0 & 3.69 & -1.51 & 78.7 & 77.5 & 57.2 \\
5293.96 & 26.0 & 4.14 & -1.77 & 57.3 & 52.5 & 29.4 \\
5295.31 & 26.0 & 4.42 & -1.59 & 53.7 & 50.8 & 29.0 \\
5307.36 & 26.0 & 1.61 & -2.97 & 114.1 & 106.4 & 82.9 \\
5389.48 & 26.0 & 4.41 & -0.45 & 109.5 & 104.9 & 82.9 \\
5395.22 & 26.0 & 4.45 & -2.07 & 44.1 & 39.4 & 20.8 \\
5398.28 & 26.0 & 4.45 & -0.63 & 96.2 & 92.9 & 71.5 \\
5409.13 & 26.0 & 4.37 & -1.06 & 83.9 & 82.0 & 54.9 \\
5432.95 & 26.0 & 4.45 & -0.94 & 94.6 & 88.5 & 68.2 \\
5441.34 & 26.0 & 4.31 & -1.63 & 61.0 & 55.8 & 31.6 \\
5461.55 & 26.0 & 4.45 & -1.8 & 55.1 & 51.2 & 26.3 \\
5464.28 & 26.0 & 4.14 & -1.58 & 63.4 & 59.4 & 38.6 \\
5466.396 & 26.0 & 4.371 & -0.565 & 107.8 & 102.8 & 76.6 \\
5466.987 & 26.0 & 3.573 & -2.23 & 63.5 & 60.4 & 34.6 \\
5470.09 & 26.0 & 4.45 & -1.71 & 53.6 & 51.1 & 25.4 \\
5472.71 & 26.0 & 4.21 & -1.52 & 82.0 & 78.2 & 44.7 \\
5483.1 & 26.0 & 4.15 & -1.45 & 70.4 & 67.9 & 46.4 \\
5487.15 & 26.0 & 4.42 & -1.43 & 60.8 & 56.4 & 34.0 \\
5491.832 & 26.0 & 4.186 & -2.188 & 34.9 & 32.5 & 12.7 \\
5501.47 & 26.0 & 0.96 & -3.06 & 174.1 & 164.8 & 113.3 \\
5525.54 & 26.0 & 4.23 & -1.12 & 84.6 & 80.7 & 54.0 \\
5543.94 & 26.0 & 4.22 & -1.04 & 89.3 & 87.1 & 61.1 \\
5546.51 & 26.0 & 4.37 & -1.21 & 82.9 & 78.2 & 52.5 \\
5554.89 & 26.0 & 4.55 & -0.36 & 144.4 & 137.1 & 96.0 \\
5560.21 & 26.0 & 4.43 & -1.09 & 77.1 & 73.7 & 51.4 \\
5577.02 & 26.0 & 5.03 & -1.543 & 27.9 & 25.0 & 10.7 \\
5600.224 & 26.0 & 4.26 & -1.42 & 64.5 & 60.2 & 37.7 \\
5618.63 & 26.0 & 4.21 & -1.27 & 74.1 & 69.1 & 49.9 \\
5624.02 & 26.0 & 4.39 & -1.38 & 82.4 & 77.3 & 50.2 \\
5633.95 & 26.0 & 4.99 & -0.23 & 93.5 & 89.0 & 65.4 \\
5635.82 & 26.0 & 4.26 & -1.79 & 59.2 & 56.5 & 33.2 \\
5636.7 & 26.0 & 3.64 & -2.51 & 43.8 & 40.1 & 19.5 \\
5638.26 & 26.0 & 4.22 & -0.77 & 110.1 & 106.1 & 76.4 \\
5649.987 & 26.0 & 5.0995 & -0.8 & 60.3 & 57.7 & 35.7 \\
5650.71 & 26.0 & 5.09 & -0.86 & 68.3 & 64.7 & 39.1 \\
5651.469 & 26.0 & 4.473 & -1.75 & 41.9 & 38.4 & 18.3 \\
5653.87 & 26.0 & 4.39 & -1.54 & 63.8 & 62.1 & 37.2 \\
5661.348 & 26.0 & 4.284 & -1.756 & 51.2 & 47.5 & 22.4 \\
5679.023 & 26.0 & 4.652 & -0.75 & 86.8 & 82.6 & 58.9 \\
5696.09 & 26.0 & 4.548 & -1.72 & 31.9 & 29.9 & 13.6 \\
5701.544 & 26.0 & 2.559 & -2.163 & 127.0 & 120.5 & 81.3 \\
5705.464 & 26.0 & 4.301 & -1.355 & 64.6 & 62.3 & 37.9 \\
5717.83 & 26.0 & 4.28 & -1.03 & 93.2 & 89.1 & 62.3 \\
5731.76 & 26.0 & 4.26 & -1.2 & 85.7 & 82.7 & 57.7 \\
5741.85 & 26.0 & 4.26 & -1.672 & 58.5 & 55.1 & 31.7 \\
5752.03 & 26.0 & 4.55 & -1.177 & 82.1 & 77.4 & 54.9 \\
5775.08 & 26.0 & 4.22 & -1.3 & 87.2 & 83.1 & 58.1 \\
5778.453 & 26.0 & 2.588 & -3.44 & 54.1 & 51.6 & 22.0 \\
5784.658 & 26.0 & 3.396 & -2.532 & 57.0 & 52.6 & 25.8 \\
5809.218 & 26.0 & 3.883 & -1.71 & 89.1 & 82.7 & 49.1 \\
5814.81 & 26.0 & 4.28 & -1.87 & 48.8 & 44.2 & 23.6 \\
5837.7 & 26.0 & 4.29 & -2.24 & 26.2 & 23.5 & 10.1 \\
5849.68 & 26.0 & 3.69 & -2.89 & 25.3 & 21.8 & 8.6 \\
5852.22 & 26.0 & 4.55 & -1.23 & 73.2 & 68.4 & 40.3 \\
5855.076 & 26.0 & 4.608 & -1.478 & 46.8 & 43.6 & 22.8 \\
5856.09 & 26.0 & 4.29 & -1.46 & 59.7 & 56.0 & 33.5 \\
5858.78 & 26.0 & 4.22 & -2.16 & 34.7 & 32.3 & 13.3 \\
5859.59 & 26.0 & 4.55 & -0.58 & 104.6 & 98.8 & 71.9 \\
5861.11 & 26.0 & 4.28 & -2.304 & 24.4 & 21.5 & 8.8 \\
5902.47 & 26.0 & 4.59 & -1.71 & 35.7 & 32.0 & 14.0 \\
5905.67 & 26.0 & 4.65 & -0.69 & 88.3 & 83.8 & 58.8 \\
5909.97 & 26.0 & 3.21 & -2.6 & 69.5 & 63.0 & 33.6 \\
5916.25 & 26.0 & 2.45 & -2.99 & 88.6 & 83.3 & 53.4 \\
5927.79 & 26.0 & 4.65 & -0.99 & 67.4 & 64.4 & 42.6 \\
5929.68 & 26.0 & 4.55 & -1.31 & 66.3 & 62.7 & 39.4 \\
5934.65 & 26.0 & 3.93 & -1.07 & 111.2 & 107.1 & 75.0 \\
5956.694 & 26.0 & 0.859 & -4.552 & 88.0 & 82.2 & 50.5 \\
5976.78 & 26.0 & 3.94 & -1.243 & 103.1 & 98.3 & 66.8 \\
5987.065 & 26.0 & 4.795 & -0.212 & 105.6 & 99.5 & 68.2 \\
6003.01 & 26.0 & 3.88 & -1.06 & 126.4 & 119.4 & 83.7 \\
6005.541 & 26.0 & 2.588 & -3.43 & 58.2 & 52.1 & 22.1 \\
6027.05 & 26.0 & 4.076 & -1.09 & 87.9 & 84.6 & 63.8 \\
6054.07 & 26.0 & 4.37 & -2.333 & 26.7 & 23.7 & 8.4 \\
6056.0 & 26.0 & 4.73 & -0.4 & 103.9 & 97.9 & 71.1 \\
6078.49 & 26.0 & 4.8 & -0.321 & 111.9 & 104.4 & 76.6 \\
6079.01 & 26.0 & 4.65 & -1.02 & 71.9 & 68.8 & 45.3 \\
6082.71 & 26.0 & 2.22 & -3.57 & 70.7 & 64.7 & 35.1 \\
6085.26 & 26.0 & 2.76 & -3.05 & 87.5 & 80.4 & 43.2 \\
6127.91 & 26.0 & 4.14 & -1.4 & 77.0 & 73.4 & 48.1 \\
6151.618 & 26.0 & 2.176 & -3.282 & 82.5 & 77.7 & 49.2 \\
6157.72 & 26.0 & 4.07 & -1.2 & 89.2 & 85.0 & 60.5 \\
6165.36 & 26.0 & 4.143 & -1.46 & 70.0 & 66.1 & 44.3 \\
6173.335 & 26.0 & 2.223 & -2.88 & 102.5 & 97.8 & 67.2 \\
6180.2 & 26.0 & 2.73 & -2.63 & 93.8 & 88.5 & 55.1 \\
6187.99 & 26.0 & 3.94 & -1.62 & 81.5 & 78.2 & 47.7 \\
6200.313 & 26.0 & 2.609 & -2.416 & 110.5 & 105.3 & 71.0 \\
6213.43 & 26.0 & 2.223 & -2.52 & 120.5 & 115.4 & 83.0 \\
6219.28 & 26.0 & 2.2 & -2.43 & 134.5 & 127.5 & 91.0 \\
6226.736 & 26.0 & 3.883 & -2.1 & 60.3 & 55.0 & 29.1 \\
6229.23 & 26.0 & 2.85 & -2.83 & 72.7 & 68.3 & 39.6 \\
6232.64 & 26.0 & 3.65 & -1.22 & 126.6 & 120.3 & 83.9 \\
6240.646 & 26.0 & 2.223 & -3.287 & 77.7 & 73.7 & 48.5 \\
6265.134 & 26.0 & 2.176 & -2.547 & 129.1 & 122.5 & 84.9 \\
6270.225 & 26.0 & 2.858 & -2.54 & 84.8 & 81.2 & 51.1 \\
6271.279 & 26.0 & 3.332 & -2.703 & 56.2 & 51.9 & 23.3 \\
6297.793 & 26.0 & 2.223 & -2.715 & 111.1 & 104.6 & 73.3 \\
6322.69 & 26.0 & 2.59 & -2.43 & 116.7 & 111.6 & 75.9 \\
6335.33 & 26.0 & 2.2 & -2.26 & 138.8 & 132.5 & 96.6 \\
6344.15 & 26.0 & 2.43 & -2.92 & 93.6 & 89.5 & 59.0 \\
6358.68 & 26.0 & 0.86 & -4.24 & 134.1 & 128.8 & 83.7 \\
6380.74 & 26.0 & 4.19 & -1.32 & 80.9 & 78.5 & 51.5 \\
6392.539 & 26.0 & 2.279 & -4.03 & 48.4 & 42.9 & 16.8 \\
6419.95 & 26.0 & 4.73 & -0.24 & 124.9 & 120.0 & 76.9 \\
6430.846 & 26.0 & 2.176 & -2.006 & 172.3 & 163.3 & 111.0 \\
6481.87 & 26.0 & 2.28 & -2.98 & 101.8 & 95.2 & 64.8 \\
6498.939 & 26.0 & 0.958 & -4.695 & 85.9 & 81.0 & 45.6 \\
6518.367 & 26.0 & 2.831 & -2.448 & 91.5 & 86.1 & 56.5 \\
6574.229 & 26.0 & 0.99 & -5.01 & 70.8 & 65.5 & 28.5 \\
6593.871 & 26.0 & 2.433 & -2.394 & 124.1 & 116.9 & 83.7 \\
6597.56 & 26.0 & 4.8 & -0.97 & 72.1 & 68.2 & 43.7 \\
6609.11 & 26.0 & 2.559 & -2.682 & 96.4 & 92.0 & 65.7 \\
6699.142 & 26.0 & 4.593 & -2.101 & 24.8 & 23.1 & 8.3 \\
6625.022 & 26.0 & 1.011 & -5.336 & 53.7 & 49.2 & 15.0 \\
6703.567 & 26.0 & 2.759 & -3.023 & 72.1 & 68.4 & 36.6 \\
6705.102 & 26.0 & 4.607 & -0.98 & 79.7 & 75.4 & 46.4 \\
6710.319 & 26.0 & 1.485 & -4.88 & 52.9 & 47.5 & 15.7 \\
6713.745 & 26.0 & 4.795 & -1.4 & 44.7 & 42.1 & 21.2 \\
6725.357 & 26.0 & 4.103 & -2.19 & 43.1 & 39.6 & 18.3 \\
6726.667 & 26.0 & 4.607 & -1.03 & 76.7 & 72.8 & 46.2 \\
6733.151 & 26.0 & 4.638 & -1.47 & 53.4 & 50.7 & 26.6 \\
6739.522 & 26.0 & 1.557 & -4.794 & 41.9 & 37.2 & 11.4 \\
6750.152 & 26.0 & 2.424 & -2.621 & 111.7 & 108.0 & 73.5 \\
6806.845 & 26.0 & 2.727 & -3.11 & 70.3 & 65.0 & 35.0 \\
6810.263 & 26.0 & 4.607 & -0.986 & 79.7 & 76.6 & 49.9 \\
6828.59 & 26.0 & 4.64 & -0.82 & 86.5 & 82.3 & 54.8 \\
6837.006 & 26.0 & 4.593 & -1.687 & 38.8 & 35.0 & 17.0 \\
6839.83 & 26.0 & 2.559 & -3.35 & 66.5 & 61.5 & 30.5 \\
6841.34 & 26.0 & 4.61 & -0.71 & 85.1 & 80.5 & 60.8 \\
6842.69 & 26.0 & 4.64 & -1.22 & 66.8 & 62.7 & 38.3 \\
6843.66 & 26.0 & 4.55 & -0.83 & 94.6 & 89.6 & 60.8 \\
6854.823 & 26.0 & 4.593 & -1.926 & 30.8 & 27.8 & 12.9 \\
6855.16 & 26.0 & 4.56 & -0.74 & 104.6 & 101.5 & 71.9 \\
6858.15 & 26.0 & 4.61 & -0.94 & 79.6 & 74.8 & 51.3 \\
7090.38 & 26.0 & 4.23 & -1.11 & 110.0 & 103.3 & 66.3 \\
7132.99 & 26.0 & 4.08 & -1.65 & 72.1 & 68.7 & 42.5 \\
7401.685 & 26.0 & 4.186 & -1.5 & 67.9 & 64.7 & 41.7 \\
7418.67 & 26.0 & 4.14 & -1.38 & 80.2 & 75.4 & 48.9 \\
7583.79 & 26.0 & 3.02 & -1.88 & 126.4 & 119.9 & 82.8 \\
7710.36 & 26.0 & 4.22 & -1.11 & 105.0 & 100.7 & 67.0 \\
7723.21 & 26.0 & 2.28 & -3.62 & 82.0 & 74.7 & 40.6 \\
4508.29 & 26.1 & 2.856 & -2.52 & 85.2 & 84.4 & 84.7 \\
4520.224 & 26.1 & 2.8068 & -2.65 & 76.3 & 75.7 & 78.6 \\
4576.333 & 26.1 & 2.844 & -2.95 & 69.1 & 69.6 & 64.4 \\
4993.34 & 26.1 & 2.81 & -3.73 & 46.1 & 45.2 & 39.1 \\
5197.577 & 26.1 & 3.231 & -2.22 & 81.0 & 81.3 & 88.4 \\
5234.624 & 26.1 & 3.221 & -2.18 & 81.1 & 81.3 & 82.4 \\
5264.804 & 26.1 & 3.23 & -3.13 & 44.6 & 44.4 & 45.1 \\
5414.072 & 26.1 & 3.221 & -3.58 & 29.7 & 29.8 & 26.7 \\
5425.257 & 26.1 & 3.2 & -3.22 & 44.8 & 46.0 & 41.1 \\
5534.84 & 26.1 & 3.24 & -2.88 & 57.6 & 57.6 & 56.0 \\
6084.09 & 26.1 & 3.2 & -3.83 & 24.8 & 24.4 & 21.3 \\
6149.24 & 26.1 & 3.89 & -2.75 & 35.8 & 35.7 & 34.9 \\
6238.38 & 26.1 & 3.89 & -2.63 & 49.7 & 48.3 & 44.3 \\
6247.55 & 26.1 & 3.89 & -2.38 & 49.6 & 49.1 & 54.1 \\
6369.462 & 26.1 & 2.891 & -4.11 & 19.9 & 20.6 & 18.6 \\
6432.676 & 26.1 & 2.891 & -3.57 & 42.3 & 41.7 & 40.9 \\
6456.383 & 26.1 & 3.9036 & -2.05 & 56.6 & 56.8 & 61.0 \\
6516.077 & 26.1 & 2.891 & -3.31 & 59.4 & 60.7 & 56.3 \\
7711.721 & 26.1 & 3.903 & -2.5 & 47.0 & 46.7 & 46.2 \\
4792.8604 & 27.0 & 3.2524 & -0.921 & 66.9 & 62.5 & 33.2 \\
-4792.7988 & 27.0 & 3.2524 & -2.734 & 0.0 & 0.0 & 0.0 \\
-4792.814 & 27.0 & 3.2524 & -2.324 & 0.0 & 0.0 & 0.0 \\
-4792.8242 & 27.0 & 3.2524 & -1.62 & 0.0 & 0.0 & 0.0 \\
-4792.8271 & 27.0 & 3.2524 & -2.102 & 0.0 & 0.0 & 0.0 \\
-4792.834 & 27.0 & 3.2524 & -1.424 & 0.0 & 0.0 & 0.0 \\
-4792.8379 & 27.0 & 3.2524 & -1.977 & 0.0 & 0.0 & 0.0 \\
-4792.8428 & 27.0 & 3.2524 & -1.37 & 0.0 & 0.0 & 0.0 \\
-4792.8477 & 27.0 & 3.2524 & -1.926 & 0.0 & 0.0 & 0.0 \\
-4792.8501 & 27.0 & 3.2524 & -1.392 & 0.0 & 0.0 & 0.0 \\
-4792.854 & 27.0 & 3.2524 & -0.78 & 0.0 & 0.0 & 0.0 \\
-4792.856 & 27.0 & 3.2524 & -1.956 & 0.0 & 0.0 & 0.0 \\
-4792.856 & 27.0 & 3.2524 & -1.483 & 0.0 & 0.0 & 0.0 \\
-4792.8604 & 27.0 & 3.2524 & -1.671 & 0.0 & 0.0 & 0.0 \\
-4792.8643 & 27.0 & 3.2524 & -1.085 & 0.0 & 0.0 & 0.0 \\
-4792.8672 & 27.0 & 3.2524 & -1.283 & 0.0 & 0.0 & 0.0 \\
-4792.8682 & 27.0 & 3.2524 & -1.926 & 0.0 & 0.0 & 0.0 \\
-4792.8682 & 27.0 & 3.2524 & -1.538 & 0.0 & 0.0 & 0.0 \\
4813.478 & 27.0 & 3.2158 & -0.601 & 84.0 & 79.0 & 44.9 \\
-4813.3979 & 27.0 & 3.2158 & -2.805 & 0.0 & 0.0 & 0.0 \\
-4813.416 & 27.0 & 3.2158 & -2.407 & 0.0 & 0.0 & 0.0 \\
-4813.4321 & 27.0 & 3.2158 & -2.203 & 0.0 & 0.0 & 0.0 \\
-4813.4321 & 27.0 & 3.2158 & -1.504 & 0.0 & 0.0 & 0.0 \\
-4813.4453 & 27.0 & 3.2158 & -1.293 & 0.0 & 0.0 & 0.0 \\
-4813.4468 & 27.0 & 3.2158 & -2.106 & 0.0 & 0.0 & 0.0 \\
-4813.4561 & 27.0 & 3.2158 & -1.22 & 0.0 & 0.0 & 0.0 \\
-4813.459 & 27.0 & 3.2158 & -2.106 & 0.0 & 0.0 & 0.0 \\
-4813.4658 & 27.0 & 3.2158 & -1.214 & 0.0 & 0.0 & 0.0 \\
-4813.4697 & 27.0 & 3.2158 & -2.261 & 0.0 & 0.0 & 0.0 \\
-4813.4712 & 27.0 & 3.2158 & -0.496 & 0.0 & 0.0 & 0.0 \\
-4813.4727 & 27.0 & 3.2158 & -1.261 & 0.0 & 0.0 & 0.0 \\
-4813.479 & 27.0 & 3.2158 & -1.366 & 0.0 & 0.0 & 0.0 \\
-4813.4829 & 27.0 & 3.2158 & -1.562 & 0.0 & 0.0 & 0.0 \\
-4813.4854 & 27.0 & 3.2158 & -0.717 & 0.0 & 0.0 & 0.0 \\
-4813.4893 & 27.0 & 3.2158 & -0.846 & 0.0 & 0.0 & 0.0 \\
-4813.4902 & 27.0 & 3.2158 & -1.629 & 0.0 & 0.0 & 0.0 \\
-4813.4922 & 27.0 & 3.2158 & -0.992 & 0.0 & 0.0 & 0.0 \\
-4813.4932 & 27.0 & 3.2158 & -1.366 & 0.0 & 0.0 & 0.0 \\
-4813.4932 & 27.0 & 3.2158 & -1.162 & 0.0 & 0.0 & 0.0 \\
5212.687 & 27.0 & 3.5144 & -1.103 & 60.4 & 53.4 & 20.6 \\
-5212.591 & 27.0 & 3.5144 & -1.882 & 0.0 & 0.0 & 0.0 \\
-5212.618 & 27.0 & 3.5144 & -1.667 & 0.0 & 0.0 & 0.0 \\
-5212.642 & 27.0 & 3.5144 & -1.59 & 0.0 & 0.0 & 0.0 \\
-5212.649 & 27.0 & 3.5144 & -0.819 & 0.0 & 0.0 & 0.0 \\
-5212.664 & 27.0 & 3.5144 & -1.579 & 0.0 & 0.0 & 0.0 \\
-5212.669 & 27.0 & 3.5144 & -0.955 & 0.0 & 0.0 & 0.0 \\
-5212.683 & 27.0 & 3.5144 & -1.622 & 0.0 & 0.0 & 0.0 \\
-5212.7 & 27.0 & 3.5144 & -1.725 & 0.0 & 0.0 & 0.0 \\
-5212.701 & 27.0 & 3.5144 & -1.262 & 0.0 & 0.0 & 0.0 \\
-5212.713 & 27.0 & 3.5144 & -1.431 & 0.0 & 0.0 & 0.0 \\
-5212.714 & 27.0 & 3.5144 & -1.946 & 0.0 & 0.0 & 0.0 \\
-5212.722 & 27.0 & 3.5144 & -1.598 & 0.0 & 0.0 & 0.0 \\
-5212.728 & 27.0 & 3.5144 & -1.882 & 0.0 & 0.0 & 0.0 \\
-5212.729 & 27.0 & 3.5144 & -1.736 & 0.0 & 0.0 & 0.0 \\
-5212.734 & 27.0 & 3.5144 & -1.75 & 0.0 & 0.0 & 0.0 \\
-5212.738 & 27.0 & 3.5144 & -1.667 & 0.0 & 0.0 & 0.0 \\
-5212.745 & 27.0 & 3.5144 & -1.59 & 0.0 & 0.0 & 0.0 \\
-5212.748 & 27.0 & 3.5144 & -1.946 & 0.0 & 0.0 & 0.0 \\
-5212.75 & 27.0 & 3.5144 & -1.579 & 0.0 & 0.0 & 0.0 \\
-5212.751 & 27.0 & 3.5144 & -1.725 & 0.0 & 0.0 & 0.0 \\
-5212.752 & 27.0 & 3.5144 & -1.622 & 0.0 & 0.0 & 0.0 \\
5247.872 & 27.0 & 1.785 & -2.71 & 60.2 & 54.7 & 17.0 \\
-5247.897 & 27.0 & 1.785 & -2.564 & 0.0 & 0.0 & 0.0 \\
-5247.936 & 27.0 & 1.785 & -2.564 & 0.0 & 0.0 & 0.0 \\
-5247.962 & 27.0 & 1.785 & -3.041 & 0.0 & 0.0 & 0.0 \\
5280.6221 & 27.0 & 3.629 & -0.808 & 52.6 & 47.2 & 19.6 \\
-5280.5322 & 27.0 & 3.629 & -3.012 & 0.0 & 0.0 & 0.0 \\
-5280.5591 & 27.0 & 3.629 & -2.614 & 0.0 & 0.0 & 0.0 \\
-5280.5659 & 27.0 & 3.629 & -1.711 & 0.0 & 0.0 & 0.0 \\
-5280.583 & 27.0 & 3.629 & -2.41 & 0.0 & 0.0 & 0.0 \\
-5280.5879 & 27.0 & 3.629 & -1.5 & 0.0 & 0.0 & 0.0 \\
-5280.603 & 27.0 & 3.629 & -2.313 & 0.0 & 0.0 & 0.0 \\
-5280.605 & 27.0 & 3.629 & -0.703 & 0.0 & 0.0 & 0.0 \\
-5280.606 & 27.0 & 3.629 & -1.427 & 0.0 & 0.0 & 0.0 \\
-5280.6201 & 27.0 & 3.629 & -2.313 & 0.0 & 0.0 & 0.0 \\
-5280.6221 & 27.0 & 3.629 & -1.421 & 0.0 & 0.0 & 0.0 \\
-5280.6343 & 27.0 & 3.629 & -2.468 & 0.0 & 0.0 & 0.0 \\
-5280.6343 & 27.0 & 3.629 & -1.468 & 0.0 & 0.0 & 0.0 \\
-5280.6348 & 27.0 & 3.629 & -0.924 & 0.0 & 0.0 & 0.0 \\
-5280.644 & 27.0 & 3.629 & -1.573 & 0.0 & 0.0 & 0.0 \\
-5280.6455 & 27.0 & 3.629 & -1.053 & 0.0 & 0.0 & 0.0 \\
-5280.6499 & 27.0 & 3.629 & -1.769 & 0.0 & 0.0 & 0.0 \\
-5280.6533 & 27.0 & 3.629 & -1.199 & 0.0 & 0.0 & 0.0 \\
-5280.6582 & 27.0 & 3.629 & -1.836 & 0.0 & 0.0 & 0.0 \\
-5280.6582 & 27.0 & 3.629 & -1.369 & 0.0 & 0.0 & 0.0 \\
-5280.6592 & 27.0 & 3.629 & -1.573 & 0.0 & 0.0 & 0.0 \\
5301.043 & 27.0 & 1.71 & -3.335 & 62.5 & 57.6 & 20.0 \\
-5301.008 & 27.0 & 1.71 & -3.335 & 0.0 & 0.0 & 0.0 \\
-5301.017 & 27.0 & 1.71 & -2.636 & 0.0 & 0.0 & 0.0 \\
-5301.026 & 27.0 & 1.71 & -3.154 & 0.0 & 0.0 & 0.0 \\
-5301.034 & 27.0 & 1.71 & -2.927 & 0.0 & 0.0 & 0.0 \\
-5301.041 & 27.0 & 1.71 & -3.123 & 0.0 & 0.0 & 0.0 \\
-5301.048 & 27.0 & 1.71 & -3.334 & 0.0 & 0.0 & 0.0 \\
-5301.052 & 27.0 & 1.71 & -3.187 & 0.0 & 0.0 & 0.0 \\
-5301.056 & 27.0 & 1.71 & -3.154 & 0.0 & 0.0 & 0.0 \\
-5301.058 & 27.0 & 1.71 & -4.051 & 0.0 & 0.0 & 0.0 \\
-5301.061 & 27.0 & 1.71 & -3.386 & 0.0 & 0.0 & 0.0 \\
-5301.065 & 27.0 & 1.71 & -5.295 & 0.0 & 0.0 & 0.0 \\
-5301.065 & 27.0 & 1.71 & -3.123 & 0.0 & 0.0 & 0.0 \\
-5301.07 & 27.0 & 1.71 & -3.641 & 0.0 & 0.0 & 0.0 \\
-5301.071 & 27.0 & 1.71 & -3.187 & 0.0 & 0.0 & 0.0 \\
-5301.074 & 27.0 & 1.71 & -3.386 & 0.0 & 0.0 & 0.0 \\
5483.354 & 27.0 & 1.7104 & -2.425 & 109.6 & 101.0 & 52.6 \\
-5483.309 & 27.0 & 1.7104 & -2.12 & 0.0 & 0.0 & 0.0 \\
-5483.334 & 27.0 & 1.7104 & -2.261 & 0.0 & 0.0 & 0.0 \\
-5483.344 & 27.0 & 1.7104 & -2.961 & 0.0 & 0.0 & 0.0 \\
-5483.363 & 27.0 & 1.7104 & -2.764 & 0.0 & 0.0 & 0.0 \\
-5483.37 & 27.0 & 1.7104 & -2.623 & 0.0 & 0.0 & 0.0 \\
-5483.372 & 27.0 & 1.7104 & -4.074 & 0.0 & 0.0 & 0.0 \\
-5483.378 & 27.0 & 1.7104 & -2.71 & 0.0 & 0.0 & 0.0 \\
-5483.383 & 27.0 & 1.7104 & -2.878 & 0.0 & 0.0 & 0.0 \\
-5483.387 & 27.0 & 1.7104 & -3.664 & 0.0 & 0.0 & 0.0 \\
-5483.389 & 27.0 & 1.7104 & -2.732 & 0.0 & 0.0 & 0.0 \\
-5483.393 & 27.0 & 1.7104 & -3.266 & 0.0 & 0.0 & 0.0 \\
-5483.397 & 27.0 & 1.7104 & -2.822 & 0.0 & 0.0 & 0.0 \\
-5483.397 & 27.0 & 1.7104 & -3.442 & 0.0 & 0.0 & 0.0 \\
-5483.402 & 27.0 & 1.7104 & -3.011 & 0.0 & 0.0 & 0.0 \\
-5483.403 & 27.0 & 1.7104 & -3.317 & 0.0 & 0.0 & 0.0 \\
-5483.407 & 27.0 & 1.7104 & -3.296 & 0.0 & 0.0 & 0.0 \\
-5483.407 & 27.0 & 1.7104 & -3.266 & 0.0 & 0.0 & 0.0 \\
5647.232 & 27.0 & 2.28 & -2.626 & 48.3 & 43.1 & 14.5 \\
-5647.207 & 27.0 & 2.28 & -2.127 & 0.0 & 0.0 & 0.0 \\
-5647.22 & 27.0 & 2.28 & -2.343 & 0.0 & 0.0 & 0.0 \\
-5647.239 & 27.0 & 2.28 & -2.753 & 0.0 & 0.0 & 0.0 \\
-5647.243 & 27.0 & 2.28 & -3.065 & 0.0 & 0.0 & 0.0 \\
-5647.246 & 27.0 & 2.28 & -2.592 & 0.0 & 0.0 & 0.0 \\
-5647.253 & 27.0 & 2.28 & -2.6 & 0.0 & 0.0 & 0.0 \\
-5647.259 & 27.0 & 2.28 & -2.764 & 0.0 & 0.0 & 0.0 \\
-5647.265 & 27.0 & 2.28 & -3.618 & 0.0 & 0.0 & 0.0 \\
-5647.267 & 27.0 & 2.28 & -3.19 & 0.0 & 0.0 & 0.0 \\
-5647.269 & 27.0 & 2.28 & -2.764 & 0.0 & 0.0 & 0.0 \\
-5647.269 & 27.0 & 2.28 & -2.94 & 0.0 & 0.0 & 0.0 \\
6082.4214 & 27.0 & 3.5144 & -1.989 & 44.1 & 40.1 & 12.7 \\
-6082.3149 & 27.0 & 3.5144 & -2.356 & 0.0 & 0.0 & 0.0 \\
-6082.3198 & 27.0 & 3.5144 & -2.135 & 0.0 & 0.0 & 0.0 \\
-6082.3247 & 27.0 & 3.5144 & -2.16 & 0.0 & 0.0 & 0.0 \\
-6082.3296 & 27.0 & 3.5144 & -2.032 & 0.0 & 0.0 & 0.0 \\
-6082.335 & 27.0 & 3.5144 & -2.146 & 0.0 & 0.0 & 0.0 \\
-6082.3447 & 27.0 & 3.5144 & -2.356 & 0.0 & 0.0 & 0.0 \\
-6082.3462 & 27.0 & 3.5144 & -1.989 & 0.0 & 0.0 & 0.0 \\
-6082.3496 & 27.0 & 3.5144 & -2.008 & 0.0 & 0.0 & 0.0 \\
-6082.3652 & 27.0 & 3.5144 & -2.135 & 0.0 & 0.0 & 0.0 \\
-6082.3657 & 27.0 & 3.5144 & -2.0 & 0.0 & 0.0 & 0.0 \\
-6082.3711 & 27.0 & 3.5144 & -1.841 & 0.0 & 0.0 & 0.0 \\
-6082.3901 & 27.0 & 3.5144 & -2.032 & 0.0 & 0.0 & 0.0 \\
-6082.3921 & 27.0 & 3.5144 & -2.077 & 0.0 & 0.0 & 0.0 \\
-6082.3965 & 27.0 & 3.5144 & -1.672 & 0.0 & 0.0 & 0.0 \\
-6082.4219 & 27.0 & 3.5144 & -2.292 & 0.0 & 0.0 & 0.0 \\
-6082.4263 & 27.0 & 3.5144 & -1.513 & 0.0 & 0.0 & 0.0 \\
-6082.4561 & 27.0 & 3.5144 & -2.0 & 0.0 & 0.0 & 0.0 \\
-6082.4609 & 27.0 & 3.5144 & -1.365 & 0.0 & 0.0 & 0.0 \\
-6082.4956 & 27.0 & 3.5144 & -2.077 & 0.0 & 0.0 & 0.0 \\
-6082.502 & 27.0 & 3.5144 & -1.229 & 0.0 & 0.0 & 0.0 \\
-6082.541 & 27.0 & 3.5144 & -2.292 & 0.0 & 0.0 & 0.0 \\
6093.1484 & 27.0 & 1.7403 & -3.468 & 40.5 & 35.8 & 10.1 \\
-6093.0952 & 27.0 & 1.7403 & -3.457 & 0.0 & 0.0 & 0.0 \\
-6093.1157 & 27.0 & 1.7403 & -3.046 & 0.0 & 0.0 & 0.0 \\
-6093.124 & 27.0 & 1.7403 & -3.343 & 0.0 & 0.0 & 0.0 \\
-6093.1392 & 27.0 & 1.7403 & -3.662 & 0.0 & 0.0 & 0.0 \\
-6093.1597 & 27.0 & 1.7403 & -3.457 & 0.0 & 0.0 & 0.0 \\
-6093.1738 & 27.0 & 1.7403 & -3.644 & 0.0 & 0.0 & 0.0 \\
-6093.1738 & 27.0 & 1.7403 & -3.343 & 0.0 & 0.0 & 0.0 \\
-6093.1846 & 27.0 & 1.7403 & -3.468 & 0.0 & 0.0 & 0.0 \\
6188.925 & 27.0 & 1.71 & -3.805 & 46.3 & 40.0 & 10.8 \\
-6188.937 & 27.0 & 1.71 & -3.106 & 0.0 & 0.0 & 0.0 \\
-6188.968 & 27.0 & 1.71 & -3.624 & 0.0 & 0.0 & 0.0 \\
-6188.979 & 27.0 & 1.71 & -3.398 & 0.0 & 0.0 & 0.0 \\
-6188.991 & 27.0 & 1.71 & -3.805 & 0.0 & 0.0 & 0.0 \\
-6189.003 & 27.0 & 1.71 & -3.593 & 0.0 & 0.0 & 0.0 \\
-6189.012 & 27.0 & 1.71 & -3.804 & 0.0 & 0.0 & 0.0 \\
-6189.024 & 27.0 & 1.71 & -3.624 & 0.0 & 0.0 & 0.0 \\
-6189.03 & 27.0 & 1.71 & -3.657 & 0.0 & 0.0 & 0.0 \\
-6189.038 & 27.0 & 1.71 & -4.521 & 0.0 & 0.0 & 0.0 \\
-6189.048 & 27.0 & 1.71 & -3.593 & 0.0 & 0.0 & 0.0 \\
-6189.052 & 27.0 & 1.71 & -3.856 & 0.0 & 0.0 & 0.0 \\
-6189.057 & 27.0 & 1.71 & -5.764 & 0.0 & 0.0 & 0.0 \\
-6189.065 & 27.0 & 1.71 & -3.657 & 0.0 & 0.0 & 0.0 \\
-6189.069 & 27.0 & 1.71 & -4.111 & 0.0 & 0.0 & 0.0 \\
-6189.075 & 27.0 & 1.71 & -3.856 & 0.0 & 0.0 & 0.0 \\
6454.946 & 27.0 & 3.632 & -1.4194 & 47.2 & 40.3 & 15.4 \\
-6454.934 & 27.0 & 3.632 & -2.0562 & 0.0 & 0.0 & 0.0 \\
-6454.944 & 27.0 & 3.632 & -1.9892 & 0.0 & 0.0 & 0.0 \\
-6454.933 & 27.0 & 3.632 & -1.7929 & 0.0 & 0.0 & 0.0 \\
-6454.965 & 27.0 & 3.632 & -2.6882 & 0.0 & 0.0 & 0.0 \\
-6454.954 & 27.0 & 3.632 & -1.7929 & 0.0 & 0.0 & 0.0 \\
-6454.937 & 27.0 & 3.632 & -1.5888 & 0.0 & 0.0 & 0.0 \\
-6454.985 & 27.0 & 3.632 & -2.5333 & 0.0 & 0.0 & 0.0 \\
-6454.968 & 27.0 & 3.632 & -1.6882 & 0.0 & 0.0 & 0.0 \\
-6455.01 & 27.0 & 3.632 & -2.5333 & 0.0 & 0.0 & 0.0 \\
-6454.987 & 27.0 & 3.632 & -1.6412 & 0.0 & 0.0 & 0.0 \\
-6454.959 & 27.0 & 3.632 & -1.2732 & 0.0 & 0.0 & 0.0 \\
-6455.04 & 27.0 & 3.632 & -2.6302 & 0.0 & 0.0 & 0.0 \\
-6455.012 & 27.0 & 3.632 & -1.6468 & 0.0 & 0.0 & 0.0 \\
-6454.978 & 27.0 & 3.632 & -1.1441 & 0.0 & 0.0 & 0.0 \\
-6455.074 & 27.0 & 3.632 & -2.8343 & 0.0 & 0.0 & 0.0 \\
-6455.041 & 27.0 & 3.632 & -1.7204 & 0.0 & 0.0 & 0.0 \\
-6455.002 & 27.0 & 3.632 & -1.0282 & 0.0 & 0.0 & 0.0 \\
-6455.114 & 27.0 & 3.632 & -3.2323 & 0.0 & 0.0 & 0.0 \\
-6455.075 & 27.0 & 3.632 & -1.9312 & 0.0 & 0.0 & 0.0 \\
-6455.03 & 27.0 & 3.632 & -0.9226 & 0.0 & 0.0 & 0.0 \\
6814.9688 & 27.0 & 1.9557 & -3.026 & 66.1 & 60.6 & 19.2 \\
-6814.8887 & 27.0 & 1.9557 & -2.839 & 0.0 & 0.0 & 0.0 \\
-6814.915 & 27.0 & 1.9557 & -2.725 & 0.0 & 0.0 & 0.0 \\
-6814.9238 & 27.0 & 1.9557 & -2.428 & 0.0 & 0.0 & 0.0 \\
-6814.936 & 27.0 & 1.9557 & -2.85 & 0.0 & 0.0 & 0.0 \\
-6814.9434 & 27.0 & 1.9557 & -3.044 & 0.0 & 0.0 & 0.0 \\
-6814.978 & 27.0 & 1.9557 & -2.839 & 0.0 & 0.0 & 0.0 \\
-6814.9873 & 27.0 & 1.9557 & -2.725 & 0.0 & 0.0 & 0.0 \\
-6814.9907 & 27.0 & 1.9557 & -2.85 & 0.0 & 0.0 & 0.0 \\
7417.3853 & 27.0 & 2.0421 & -3.263 & 49.7 & 41.7 & 11.8 \\
-7417.3076 & 27.0 & 2.0421 & -2.637 & 0.0 & 0.0 & 0.0 \\
-7417.3491 & 27.0 & 2.0421 & -2.853 & 0.0 & 0.0 & 0.0 \\
-7417.3838 & 27.0 & 2.0421 & -3.136 & 0.0 & 0.0 & 0.0 \\
-7417.4126 & 27.0 & 2.0421 & -3.102 & 0.0 & 0.0 & 0.0 \\
-7417.4141 & 27.0 & 2.0421 & -3.575 & 0.0 & 0.0 & 0.0 \\
-7417.4355 & 27.0 & 2.0421 & -3.11 & 0.0 & 0.0 & 0.0 \\
-7417.4487 & 27.0 & 2.0421 & -4.128 & 0.0 & 0.0 & 0.0 \\
-7417.4517 & 27.0 & 2.0421 & -3.274 & 0.0 & 0.0 & 0.0 \\
-7417.4639 & 27.0 & 2.0421 & -3.7 & 0.0 & 0.0 & 0.0 \\
-7417.4736 & 27.0 & 2.0421 & -3.45 & 0.0 & 0.0 & 0.0 \\
-7417.4766 & 27.0 & 2.0421 & -3.274 & 0.0 & 0.0 & 0.0 \\
4814.5979 & 28.0 & 3.597 & -1.62 & 32.5 & 29.1 & 15.3 \\
4831.18 & 28.0 & 3.61 & -0.32 & 97.8 & 93.3 & 74.0 \\
4853.78 & 28.0 & 3.543 & -1.55 & 48.3 & 45.3 & 21.3 \\
4866.27 & 28.0 & 3.539 & -0.21 & 99.6 & 94.1 & 74.9 \\
4874.7929 & 28.0 & 3.543 & -1.45 & 53.9 & 48.4 & 26.2 \\
4886.7108 & 28.0 & 3.706 & -1.78 & 31.4 & 28.3 & 13.7 \\
4904.42 & 28.0 & 3.54 & -0.25 & 125.2 & 115.4 & 85.9 \\
4913.98 & 28.0 & 3.74 & -0.661 & 79.4 & 75.1 & 54.6 \\
4946.04 & 28.0 & 3.8 & -1.224 & 56.1 & 53.1 & 27.6 \\
4952.29 & 28.0 & 3.61 & -1.261 & 63.8 & 59.2 & 32.4 \\
4953.21 & 28.0 & 3.74 & -0.58 & 82.1 & 78.8 & 55.0 \\
4976.1348 & 28.0 & 3.606 & -1.25 & 56.7 & 52.0 & 31.0 \\
4995.66 & 28.0 & 3.63 & -1.611 & 33.9 & 33.5 & 14.6 \\
4998.22 & 28.0 & 3.606 & -0.69 & 74.3 & 71.7 & 52.2 \\
5010.94 & 28.0 & 3.63 & -0.901 & 65.1 & 62.9 & 48.4 \\
5081.11 & 28.0 & 3.85 & 0.064 & 113.4 & 109.6 & 91.8 \\
5082.35 & 28.0 & 3.658 & -0.59 & 90.8 & 87.2 & 65.3 \\
5084.11 & 28.0 & 3.68 & -0.06 & 118.5 & 114.8 & 89.0 \\
5088.96 & 28.0 & 3.68 & -1.29 & 51.1 & 49.2 & 26.0 \\
5094.42 & 28.0 & 3.833 & -1.07 & 50.1 & 46.9 & 29.0 \\
5102.97 & 28.0 & 1.68 & -2.66 & 82.4 & 80.7 & 49.4 \\
5115.4 & 28.0 & 3.834 & -0.28 & 90.3 & 87.2 & 69.9 \\
5157.9805 & 28.0 & 3.606 & -1.51 & 38.7 & 36.5 & 18.7 \\
5392.33 & 28.0 & 4.15 & -1.32 & 28.1 & 26.8 & 13.0 \\
5435.86 & 28.0 & 1.99 & -2.432 & 85.5 & 81.8 & 52.5 \\
5462.5 & 28.0 & 3.85 & -0.88 & 73.2 & 69.6 & 42.9 \\
5468.11 & 28.0 & 3.85 & -1.66 & 31.2 & 28.2 & 12.6 \\
5578.729 & 28.0 & 1.677 & -2.57 & 89.0 & 84.2 & 54.0 \\
5587.87 & 28.0 & 1.93 & -2.44 & 75.9 & 73.7 & 54.5 \\
5589.36 & 28.0 & 3.9 & -1.148 & 48.6 & 47.7 & 26.4 \\
5593.746 & 28.0 & 3.899 & -0.78 & 69.2 & 69.0 & 43.2 \\
5625.32 & 28.0 & 4.09 & -0.731 & 61.2 & 58.0 & 39.4 \\
5628.35 & 28.0 & 4.09 & -1.316 & 33.4 & 31.0 & 14.3 \\
5638.75 & 28.0 & 3.9 & -1.699 & 24.7 & 22.1 & 8.6 \\
5641.88 & 28.0 & 4.11 & -1.017 & 49.0 & 45.6 & 23.6 \\
5643.08 & 28.0 & 4.16 & -1.234 & 34.5 & 32.5 & 14.4 \\
5694.99 & 28.0 & 4.09 & -0.629 & 65.7 & 62.5 & 42.1 \\
5748.36 & 28.0 & 1.68 & -3.24 & 61.6 & 56.5 & 28.2 \\
5749.3039 & 28.0 & 3.941 & -2.112 & 18.8 & 16.8 & 6.0 \\
-5749.2795 & 28.0 & 3.941 & -2.526 & 0.0 & 0.0 & 0.0 \\
5754.67 & 28.0 & 1.93 & -1.85 & 116.2 & 111.1 & 68.0 \\
5805.22 & 28.0 & 4.168 & -0.62 & 67.7 & 63.5 & 41.2 \\
5847.01 & 28.0 & 1.676 & -3.41 & 59.0 & 53.2 & 23.7 \\
5996.74 & 28.0 & 4.236 & -1.01 & 42.9 & 41.8 & 20.2 \\
6007.317 & 28.0 & 1.677 & -3.41 & 54.3 & 49.1 & 25.4 \\
6086.288 & 28.0 & 4.266 & -0.46 & 68.7 & 65.8 & 43.0 \\
6108.12 & 28.0 & 1.68 & -2.43 & 100.1 & 96.3 & 65.5 \\
6111.08 & 28.0 & 4.088 & -0.81 & 59.6 & 57.6 & 34.2 \\
6119.76 & 28.0 & 4.27 & -1.316 & 29.4 & 26.6 & 12.1 \\
6128.984 & 28.0 & 1.677 & -3.36 & 57.8 & 54.6 & 25.8 \\
6130.14 & 28.0 & 4.266 & -0.94 & 42.2 & 39.1 & 21.6 \\
6175.37 & 28.0 & 4.089 & -0.55 & 71.1 & 68.6 & 46.9 \\
6176.798 & 28.0 & 4.088 & -0.26 & 93.9 & 90.3 & 64.1 \\
6177.25 & 28.0 & 1.826 & -3.51 & 40.4 & 37.2 & 14.1 \\
6186.717 & 28.0 & 4.106 & -0.88 & 59.1 & 55.3 & 31.2 \\
6204.6048 & 28.0 & 4.088 & -1.1 & 48.7 & 45.5 & 23.2 \\
6223.9914 & 28.0 & 4.105 & -1.052 & 50.8 & 47.3 & 28.3 \\
-6223.971 & 28.0 & 4.105 & -1.466 & 0.0 & 0.0 & 0.0 \\
6230.1 & 28.0 & 4.11 & -1.132 & 37.4 & 33.8 & 18.9 \\
6314.668 & 28.0 & 1.936 & -2.0 & 110.3 & 104.1 & 74.2 \\
6322.169 & 28.0 & 4.154 & -1.21 & 38.6 & 36.5 & 18.3 \\
6327.6 & 28.0 & 1.68 & -3.06 & 76.0 & 72.5 & 38.5 \\
6360.81 & 28.0 & 4.17 & -1.145 & 41.2 & 36.7 & 18.4 \\
6378.258 & 28.0 & 4.154 & -0.972 & 61.9 & 58.9 & 32.3 \\
-6378.2328 & 28.0 & 4.154 & -1.386 & 0.0 & 0.0 & 0.0 \\
6482.81 & 28.0 & 1.93 & -2.76 & 82.9 & 77.9 & 41.3 \\
6598.611 & 28.0 & 4.236 & -0.91 & 47.3 & 44.1 & 24.4 \\
6635.13 & 28.0 & 4.42 & -0.72 & 51.2 & 46.0 & 25.2 \\
6643.64 & 28.0 & 1.676 & -2.03 & 133.6 & 129.5 & 92.6 \\
6767.78 & 28.0 & 1.83 & -2.1 & 110.8 & 106.9 & 77.9 \\
6772.32 & 28.0 & 3.658 & -0.97 & 73.4 & 70.2 & 48.0 \\
6813.61 & 28.0 & 5.34 & -0.33 & 24.7 & 22.0 & 11.3 \\
6842.043 & 28.0 & 3.658 & -1.5 & 48.8 & 45.8 & 25.4 \\
7110.9 & 28.0 & 1.94 & -2.88 & 91.3 & 86.9 & 38.6 \\
7715.591 & 28.0 & 3.7 & -1.01 & 80.5 & 75.8 & 51.3 \\
7748.89 & 28.0 & 3.7 & -0.38 & 122.5 & 117.6 & 85.1 \\
7788.93 & 28.0 & 1.95 & -1.75 & 146.1 & 136.7 & 92.5 \\
5105.558 & 29.0 & 1.39 & -2.102 & 140.9 & 136.1 & 93.3 \\
-5105.505 & 29.0 & 1.39 & -3.88 & 0.0 & 0.0 & 0.0 \\
-5105.509 & 29.0 & 1.39 & -2.926 & 0.0 & 0.0 & 0.0 \\
-5105.511 & 29.0 & 1.39 & -2.88 & 0.0 & 0.0 & 0.0 \\
-5105.512 & 29.0 & 1.39 & -4.056 & 0.0 & 0.0 & 0.0 \\
-5105.517 & 29.0 & 1.39 & -2.813 & 0.0 & 0.0 & 0.0 \\
-5105.52 & 29.0 & 1.39 & -2.558 & 0.0 & 0.0 & 0.0 \\
-5105.531 & 29.0 & 1.39 & -2.91 & 0.0 & 0.0 & 0.0 \\
-5105.536 & 29.0 & 1.39 & -2.308 & 0.0 & 0.0 & 0.0 \\
-5105.503 & 29.0 & 1.39 & -4.232 & 0.0 & 0.0 & 0.0 \\
-5105.506 & 29.0 & 1.39 & -3.277 & 0.0 & 0.0 & 0.0 \\
-5105.509 & 29.0 & 1.39 & -3.232 & 0.0 & 0.0 & 0.0 \\
-5105.51 & 29.0 & 1.39 & -4.408 & 0.0 & 0.0 & 0.0 \\
-5105.515 & 29.0 & 1.39 & -3.165 & 0.0 & 0.0 & 0.0 \\
-5105.519 & 29.0 & 1.39 & -2.909 & 0.0 & 0.0 & 0.0 \\
-5105.53 & 29.0 & 1.39 & -3.262 & 0.0 & 0.0 & 0.0 \\
-5105.536 & 29.0 & 1.39 & -2.659 & 0.0 & 0.0 & 0.0 \\
-5105.56 & 29.0 & 1.39 & -2.453 & 0.0 & 0.0 & 0.0 \\
5218.202 & 29.0 & 3.816 & -0.316 & 82.2 & 76.6 & 51.4 \\
-5218.191 & 29.0 & 3.816 & -1.094 & 0.0 & 0.0 & 0.0 \\
-5218.193 & 29.0 & 3.816 & -1.14 & 0.0 & 0.0 & 0.0 \\
-5218.193 & 29.0 & 3.816 & -0.772 & 0.0 & 0.0 & 0.0 \\
-5218.196 & 29.0 & 3.816 & -2.094 & 0.0 & 0.0 & 0.0 \\
-5218.196 & 29.0 & 3.816 & -1.027 & 0.0 & 0.0 & 0.0 \\
-5218.196 & 29.0 & 3.816 & -0.522 & 0.0 & 0.0 & 0.0 \\
-5218.202 & 29.0 & 3.816 & -2.27 & 0.0 & 0.0 & 0.0 \\
-5218.202 & 29.0 & 3.816 & -1.124 & 0.0 & 0.0 & 0.0 \\
-5218.19 & 29.0 & 3.816 & -1.446 & 0.0 & 0.0 & 0.0 \\
-5218.192 & 29.0 & 3.816 & -1.491 & 0.0 & 0.0 & 0.0 \\
-5218.192 & 29.0 & 3.816 & -1.123 & 0.0 & 0.0 & 0.0 \\
-5218.196 & 29.0 & 3.816 & -2.446 & 0.0 & 0.0 & 0.0 \\
-5218.196 & 29.0 & 3.816 & -1.379 & 0.0 & 0.0 & 0.0 \\
-5218.196 & 29.0 & 3.816 & -0.874 & 0.0 & 0.0 & 0.0 \\
-5218.202 & 29.0 & 3.816 & -2.622 & 0.0 & 0.0 & 0.0 \\
-5218.202 & 29.0 & 3.816 & -1.475 & 0.0 & 0.0 & 0.0 \\
-5218.202 & 29.0 & 3.816 & -0.667 & 0.0 & 0.0 & 0.0 \\
5220.065 & 29.0 & 3.816 & -1.8131 & 38.8 & 36.3 & 17.1 \\
-5220.067 & 29.0 & 3.816 & -1.8131 & 0.0 & 0.0 & 0.0 \\
-5220.066 & 29.0 & 3.816 & -2.2111 & 0.0 & 0.0 & 0.0 \\
-5220.064 & 29.0 & 3.816 & -1.609 & 0.0 & 0.0 & 0.0 \\
-5220.068 & 29.0 & 3.816 & -1.609 & 0.0 & 0.0 & 0.0 \\
-5220.066 & 29.0 & 3.816 & -1.5121 & 0.0 & 0.0 & 0.0 \\
-5220.063 & 29.0 & 3.816 & -1.667 & 0.0 & 0.0 & 0.0 \\
-5220.069 & 29.0 & 3.816 & -1.667 & 0.0 & 0.0 & 0.0 \\
-5220.066 & 29.0 & 3.816 & -1.0649 & 0.0 & 0.0 & 0.0 \\
-5220.099 & 29.0 & 3.816 & -2.1611 & 0.0 & 0.0 & 0.0 \\
-5220.101 & 29.0 & 3.816 & -2.1611 & 0.0 & 0.0 & 0.0 \\
-5220.1 & 29.0 & 3.816 & -2.5591 & 0.0 & 0.0 & 0.0 \\
-5220.098 & 29.0 & 3.816 & -1.957 & 0.0 & 0.0 & 0.0 \\
-5220.102 & 29.0 & 3.816 & -1.957 & 0.0 & 0.0 & 0.0 \\
-5220.1 & 29.0 & 3.816 & -1.8601 & 0.0 & 0.0 & 0.0 \\
-5220.097 & 29.0 & 3.816 & -2.015 & 0.0 & 0.0 & 0.0 \\
-5220.103 & 29.0 & 3.816 & -2.015 & 0.0 & 0.0 & 0.0 \\
-5220.1 & 29.0 & 3.816 & -1.4129 & 0.0 & 0.0 & 0.0 \\
7933.131 & 29.0 & 3.79 & -2.082 & 77.4 & 74.5 & 28.9 \\
-7933.092 & 29.0 & 3.79 & -1.383 & 0.0 & 0.0 & 0.0 \\
-7933.101 & 29.0 & 3.79 & -1.035 & 0.0 & 0.0 & 0.0 \\
-7933.115 & 29.0 & 3.79 & -1.383 & 0.0 & 0.0 & 0.0 \\
-7933.122 & 29.0 & 3.79 & -1.035 & 0.0 & 0.0 & 0.0 \\
-7933.136 & 29.0 & 3.79 & -1.734 & 0.0 & 0.0 & 0.0 \\
-7933.154 & 29.0 & 3.79 & -1.383 & 0.0 & 0.0 & 0.0 \\
-7933.157 & 29.0 & 3.79 & -1.035 & 0.0 & 0.0 & 0.0 \\
8092.6289 & 29.0 & 3.8167 & -0.561 & 109.7 & 106.8 & 42.7 \\
-8092.6001 & 29.0 & 3.8167 & -2.055 & 0.0 & 0.0 & 0.0 \\
-8092.6079 & 29.0 & 3.8167 & -1.707 & 0.0 & 0.0 & 0.0 \\
-8092.6079 & 29.0 & 3.8167 & -1.356 & 0.0 & 0.0 & 0.0 \\
-8092.6172 & 29.0 & 3.8167 & -1.008 & 0.0 & 0.0 & 0.0 \\
-8092.623 & 29.0 & 3.8167 & -0.909 & 0.0 & 0.0 & 0.0 \\
-8092.6362 & 29.0 & 3.8167 & -1.754 & 0.0 & 0.0 & 0.0 \\
-8092.6396 & 29.0 & 3.8167 & -1.406 & 0.0 & 0.0 & 0.0 \\
-8092.6396 & 29.0 & 3.8167 & -1.356 & 0.0 & 0.0 & 0.0 \\
-8092.644 & 29.0 & 3.8167 & -1.008 & 0.0 & 0.0 & 0.0 \\
-8092.6489 & 29.0 & 3.8167 & -1.356 & 0.0 & 0.0 & 0.0 \\
-8092.6538 & 29.0 & 3.8167 & -1.008 & 0.0 & 0.0 & 0.0 \\
4722.159 & 30.0 & 4.03 & -0.38 & 81.7 & 82.5 & 67.0 \\
4810.534 & 30.0 & 4.08 & -0.16 & 80.1 & 80.9 & 71.9 \\
6362.347 & 30.0 & 5.8 & 0.14 & 31.6 & 32.3 & 21.3 \\
7800.321 & 37.0 & 0.0 & -0.616 & 27.6 & 25.1 & 9.8 \\
-7800.293 & 37.0 & 0.0 & -0.838 & 0.0 & 0.0 & 0.0 \\
-7800.232 & 37.0 & 0.0 & -0.231 & 0.0 & 0.0 & 0.0 \\
-7800.176 & 37.0 & 0.0 & -0.378 & 0.0 & 0.0 & 0.0 \\
7947.657 & 37.0 & 0.0 & -0.924 & 15.1 & 12.7 & -- \\
-7947.629 & 37.0 & 0.0 & -1.146 & 0.0 & 0.0 & -- \\
-7947.565 & 37.0 & 0.0 & -0.539 & 0.0 & 0.0 & -- \\
-7947.513 & 37.0 & 0.0 & -0.686 & 0.0 & 0.0 & -- \\
4854.867 & 39.1 & 0.9923 & -0.857 & 60.1 & 59.1 & 46.5 \\
-4854.867 & 39.1 & 0.9923 & -0.602 & 0.0 & 0.0 & 0.0 \\
-4854.868 & 39.1 & 0.9923 & -1.556 & 0.0 & 0.0 & 0.0 \\
4883.685 & 39.1 & 1.0841 & -0.298 & 61.2 & 58.7 & 56.3 \\
-4883.685 & 39.1 & 1.0841 & -1.729 & 0.0 & 0.0 & 0.0 \\
-4883.685 & 39.1 & 1.0841 & -0.185 & 0.0 & 0.0 & 0.0 \\
4900.11 & 39.1 & 1.0326 & -0.488 & 63.6 & 60.0 & 56.4 \\
-4900.11 & 39.1 & 1.0326 & -1.634 & 0.0 & 0.0 & 0.0 \\
-4900.11 & 39.1 & 1.0326 & -0.333 & 0.0 & 0.0 & 0.0 \\
5087.418 & 39.1 & 1.0841 & -0.534 & 52.2 & 51.3 & 46.6 \\
-5087.418 & 39.1 & 1.0841 & -2.078 & 0.0 & 0.0 & 0.0 \\
-5087.42 & 39.1 & 1.0841 & -2.078 & 0.0 & 0.0 & 0.0 \\
-5087.42 & 39.1 & 1.0841 & -0.435 & 0.0 & 0.0 & 0.0 \\
5200.411 & 39.1 & 0.9923 & -1.968 & 55.9 & 51.5 & 39.0 \\
-5200.413 & 39.1 & 0.9923 & -1.014 & 0.0 & 0.0 & 0.0 \\
-5200.413 & 39.1 & 0.9923 & -0.822 & 0.0 & 0.0 & 0.0 \\
-5200.414 & 39.1 & 0.9923 & -1.968 & 0.0 & 0.0 & 0.0 \\
5402.7729 & 39.1 & 1.839 & -1.984 & 18.4 & 16.5 & 11.5 \\
-5402.7739 & 39.1 & 1.839 & -0.838 & 0.0 & 0.0 & 0.0 \\
-5402.7754 & 39.1 & 1.839 & -0.683 & 0.0 & 0.0 & 0.0 \\
5112.28 & 40.1 & 1.66 & -0.59 & 9.9 & 8.2 & 7.9 \\
5853.696 & 56.1 & 0.604 & -2.915 & 67.3 & 65.6 & 61.3 \\
-5853.697 & 56.1 & 0.604 & -2.857 & 0.0 & 0.0 & 0.0 \\
-5853.697 & 56.1 & 0.604 & -3.148 & 0.0 & 0.0 & 0.0 \\
-5853.698 & 56.1 & 0.604 & -3.09 & 0.0 & 0.0 & 0.0 \\
-5853.699 & 56.1 & 0.604 & -3.295 & 0.0 & 0.0 & 0.0 \\
-5853.699 & 56.1 & 0.604 & -3.061 & 0.0 & 0.0 & 0.0 \\
-5853.7 & 56.1 & 0.604 & -2.76 & 0.0 & 0.0 & 0.0 \\
-5853.7 & 56.1 & 0.604 & -3.693 & 0.0 & 0.0 & 0.0 \\
-5853.7 & 56.1 & 0.604 & -2.546 & 0.0 & 0.0 & 0.0 \\
-5853.7 & 56.1 & 0.604 & -2.53 & 0.0 & 0.0 & 0.0 \\
-5853.7 & 56.1 & 0.604 & -3.459 & 0.0 & 0.0 & 0.0 \\
-5853.7 & 56.1 & 0.604 & -2.313 & 0.0 & 0.0 & 0.0 \\
-5853.7 & 56.1 & 0.604 & -1.054 & 0.0 & 0.0 & 0.0 \\
-5853.7 & 56.1 & 0.604 & -2.012 & 0.0 & 0.0 & 0.0 \\
-5853.7 & 56.1 & 0.604 & -2.994 & 0.0 & 0.0 & 0.0 \\
-5853.701 & 56.1 & 0.604 & -3.295 & 0.0 & 0.0 & 0.0 \\
-5853.702 & 56.1 & 0.604 & -3.061 & 0.0 & 0.0 & 0.0 \\
-5853.703 & 56.1 & 0.604 & -2.857 & 0.0 & 0.0 & 0.0 \\
-5853.703 & 56.1 & 0.604 & -3.09 & 0.0 & 0.0 & 0.0 \\
-5853.704 & 56.1 & 0.604 & -3.148 & 0.0 & 0.0 & 0.0 \\
-5853.704 & 56.1 & 0.604 & -2.915 & 0.0 & 0.0 & 0.0 \\
6141.695 & 56.1 & 0.704 & -3.641 & 131.3 & 126.2 & 112.7 \\
-6141.695 & 56.1 & 0.704 & -3.407 & 0.0 & 0.0 & 0.0 \\
-6141.697 & 56.1 & 0.704 & -2.495 & 0.0 & 0.0 & 0.0 \\
-6141.697 & 56.1 & 0.704 & -2.261 & 0.0 & 0.0 & 0.0 \\
-6141.698 & 56.1 & 0.704 & -3.465 & 0.0 & 0.0 & 0.0 \\
-6141.698 & 56.1 & 0.704 & -3.231 & 0.0 & 0.0 & 0.0 \\
-6141.699 & 56.1 & 0.704 & -1.686 & 0.0 & 0.0 & 0.0 \\
-6141.699 & 56.1 & 0.704 & -1.453 & 0.0 & 0.0 & 0.0 \\
-6141.699 & 56.1 & 0.704 & -2.398 & 0.0 & 0.0 & 0.0 \\
-6141.699 & 56.1 & 0.704 & -2.164 & 0.0 & 0.0 & 0.0 \\
-6141.7 & 56.1 & 0.704 & -1.7 & 0.0 & 0.0 & 0.0 \\
-6141.7 & 56.1 & 0.704 & -0.224 & 0.0 & 0.0 & 0.0 \\
-6141.7 & 56.1 & 0.704 & -1.182 & 0.0 & 0.0 & 0.0 \\
-6141.701 & 56.1 & 0.704 & -1.892 & 0.0 & 0.0 & 0.0 \\
-6141.701 & 56.1 & 0.704 & -1.659 & 0.0 & 0.0 & 0.0 \\
-6141.701 & 56.1 & 0.704 & -2.51 & 0.0 & 0.0 & 0.0 \\
-6141.701 & 56.1 & 0.704 & -2.277 & 0.0 & 0.0 & 0.0 \\
-6141.702 & 56.1 & 0.704 & -1.909 & 0.0 & 0.0 & 0.0 \\
-6141.702 & 56.1 & 0.704 & -2.465 & 0.0 & 0.0 & 0.0 \\
-6141.702 & 56.1 & 0.704 & -2.143 & 0.0 & 0.0 & 0.0 \\
-6141.703 & 56.1 & 0.704 & -2.231 & 0.0 & 0.0 & 0.0 \\
6496.9 & 56.1 & 0.604 & -2.0 & 114.2 & 107.8 & 98.5 \\
-6496.906 & 56.1 & 0.604 & -2.764 & 0.0 & 0.0 & 0.0 \\
-6496.907 & 56.1 & 0.604 & -2.367 & 0.0 & 0.0 & 0.0 \\
-6496.889 & 56.1 & 0.604 & -3.066 & 0.0 & 0.0 & 0.0 \\
-6496.91 & 56.1 & 0.604 & -2.367 & 0.0 & 0.0 & 0.0 \\
-6496.892 & 56.1 & 0.604 & -2.367 & 0.0 & 0.0 & 0.0 \\
-6496.896 & 56.1 & 0.604 & -1.919 & 0.0 & 0.0 & 0.0 \\
-6496.9 & 56.1 & 0.604 & -1.482 & 0.0 & 0.0 & 0.0 \\
-6496.906 & 56.1 & 0.604 & -2.531 & 0.0 & 0.0 & 0.0 \\
-6496.908 & 56.1 & 0.604 & -2.133 & 0.0 & 0.0 & 0.0 \\
-6496.888 & 56.1 & 0.604 & -2.832 & 0.0 & 0.0 & 0.0 \\
-6496.912 & 56.1 & 0.604 & -2.133 & 0.0 & 0.0 & 0.0 \\
-6496.891 & 56.1 & 0.604 & -2.133 & 0.0 & 0.0 & 0.0 \\
-6496.896 & 56.1 & 0.604 & -1.686 & 0.0 & 0.0 & 0.0 \\
-6496.9 & 56.1 & 0.604 & -0.524 & 0.0 & 0.0 & 0.0 \\
4365.896 & 26.0 & 2.99 & -2.25 & 68.4 & 67.0 & 50.0 \\
4389.245 & 26.0 & 0.052 & -4.583 & 99.4 & 95.3 & 70.9 \\
4445.471 & 26.0 & 0.087 & -5.441 & 76.7 & 72.2 & 40.3 \\
4602.001 & 26.0 & 1.608 & -3.154 & 100.3 & 95.6 & 71.1 \\
4630.12 & 26.0 & 2.28 & -2.52 & 103.0 & 97.3 & 72.4 \\
4635.85 & 26.0 & 2.85 & -2.34 & 75.4 & 72.1 & 54.0 \\
4683.56 & 26.0 & 2.83 & -2.41 & 83.3 & 80.3 & 53.8 \\
4690.14 & 26.0 & 3.69 & -1.61 & 85.8 & 83.6 & 58.7 \\
4749.95 & 26.0 & 4.56 & -1.24 & 60.4 & 57.8 & 35.9 \\
4779.439 & 26.0 & 3.415 & -2.02 & 61.9 & 60.3 & 39.2 \\
4779.44 & 26.0 & 3.42 & -2.16 & 61.9 & 60.3 & 39.2 \\
4788.76 & 26.0 & 3.24 & -1.73 & 90.8 & 88.3 & 66.4 \\
4799.41 & 26.0 & 3.64 & -2.13 & 56.9 & 54.9 & 34.2 \\
4802.88 & 26.0 & 3.64 & -1.514 & 81.4 & 79.3 & 60.1 \\
4808.15 & 26.0 & 3.25 & -2.69 & 53.0 & 49.5 & 26.3 \\
4950.1 & 26.0 & 3.42 & -1.56 & 102.6 & 99.5 & 72.0 \\
4961.91 & 26.0 & 3.63 & -2.19 & 56.7 & 52.3 & 26.4 \\
4994.129 & 26.0 & 0.915 & -3.08 & 147.6 & 137.8 & 104.7 \\
5016.48 & 26.0 & 4.26 & -1.373 & 58.7 & 54.9 & 33.0 \\
5044.211 & 26.0 & 2.851 & -2.058 & 108.5 & 103.1 & 72.5 \\
5054.64 & 26.0 & 3.64 & -1.98 & 69.8 & 67.8 & 39.4 \\
5109.65 & 26.0 & 4.3 & -0.73 & 110.0 & 104.6 & 74.6 \\
5127.679 & 26.0 & 0.052 & -6.125 & 53.9 & 49.7 & 18.3 \\
5141.74 & 26.0 & 2.42 & -2.23 & 126.9 & 122.2 & 82.5 \\
5197.94 & 26.0 & 4.3 & -1.54 & 61.9 & 59.1 & 36.0 \\
5198.71 & 26.0 & 2.22 & -2.14 & 144.4 & 136.2 & 95.3 \\
5223.18 & 26.0 & 3.64 & -1.783 & 54.8 & 51.9 & 28.0 \\
5225.525 & 26.0 & 0.11 & -4.789 & 109.6 & 104.3 & 72.3 \\
5228.38 & 26.0 & 4.22 & -1.19 & 80.4 & 77.3 & 56.0 \\
5242.49 & 26.0 & 3.63 & -0.99 & 113.5 & 109.6 & 84.4 \\
5243.77 & 26.0 & 4.26 & -0.99 & 91.0 & 86.4 & 61.7 \\
5247.05 & 26.0 & 0.087 & -4.961 & 100.6 & 95.6 & 64.5 \\
5250.208 & 26.0 & 0.121 & -4.938 & 100.7 & 96.5 & 65.4 \\
5253.02 & 26.0 & 2.28 & -3.84 & 47.6 & 42.8 & 17.9 \\
5285.13 & 26.0 & 4.43 & -1.54 & 50.0 & 47.6 & 26.3 \\
5288.52 & 26.0 & 3.69 & -1.51 & 78.7 & 77.5 & 57.2 \\
5293.96 & 26.0 & 4.14 & -1.77 & 57.3 & 52.5 & 29.4 \\
5295.31 & 26.0 & 4.42 & -1.59 & 53.7 & 50.8 & 29.0 \\
5307.36 & 26.0 & 1.61 & -2.97 & 114.1 & 106.4 & 82.9 \\
5389.48 & 26.0 & 4.41 & -0.45 & 109.5 & 104.9 & 82.9 \\
5395.22 & 26.0 & 4.45 & -2.07 & 44.1 & 39.4 & 20.8 \\
5398.28 & 26.0 & 4.45 & -0.63 & 96.2 & 92.9 & 71.5 \\
5409.13 & 26.0 & 4.37 & -1.06 & 83.9 & 82.0 & 54.9 \\
5432.95 & 26.0 & 4.45 & -0.94 & 94.6 & 88.5 & 68.2 \\
5441.34 & 26.0 & 4.31 & -1.63 & 61.0 & 55.8 & 31.6 \\
5461.55 & 26.0 & 4.45 & -1.8 & 55.1 & 51.2 & 26.3 \\
5464.28 & 26.0 & 4.14 & -1.58 & 63.4 & 59.4 & 38.6 \\
5466.396 & 26.0 & 4.371 & -0.565 & 107.8 & 102.8 & 76.6 \\
5466.987 & 26.0 & 3.573 & -2.23 & 63.5 & 60.4 & 34.6 \\
5470.09 & 26.0 & 4.45 & -1.71 & 53.6 & 51.1 & 25.4 \\
5472.71 & 26.0 & 4.21 & -1.52 & 82.0 & 78.2 & 44.7 \\
5483.1 & 26.0 & 4.15 & -1.45 & 70.4 & 67.9 & 46.4 \\
5487.15 & 26.0 & 4.42 & -1.43 & 60.8 & 56.4 & 34.0 \\
5491.832 & 26.0 & 4.186 & -2.188 & 34.9 & 32.5 & 12.7 \\
5501.47 & 26.0 & 0.96 & -3.06 & 174.1 & 164.8 & 113.3 \\
5525.54 & 26.0 & 4.23 & -1.12 & 84.6 & 80.7 & 54.0 \\
5543.94 & 26.0 & 4.22 & -1.04 & 89.3 & 87.1 & 61.1 \\
5546.51 & 26.0 & 4.37 & -1.21 & 82.9 & 78.2 & 52.5 \\
5554.89 & 26.0 & 4.55 & -0.36 & 144.4 & 137.1 & 96.0 \\
5560.21 & 26.0 & 4.43 & -1.09 & 77.1 & 73.7 & 51.4 \\
5577.02 & 26.0 & 5.03 & -1.543 & 27.9 & 25.0 & 10.7 \\
5600.224 & 26.0 & 4.26 & -1.42 & 64.5 & 60.2 & 37.7 \\
5618.63 & 26.0 & 4.21 & -1.27 & 74.1 & 69.1 & 49.9 \\
5624.02 & 26.0 & 4.39 & -1.38 & 82.4 & 77.3 & 50.2 \\
5633.95 & 26.0 & 4.99 & -0.23 & 93.5 & 89.0 & 65.4 \\
5635.82 & 26.0 & 4.26 & -1.79 & 59.2 & 56.5 & 33.2 \\
5636.7 & 26.0 & 3.64 & -2.51 & 43.8 & 40.1 & 19.5 \\
5638.26 & 26.0 & 4.22 & -0.77 & 110.1 & 106.1 & 76.4 \\
5649.987 & 26.0 & 5.0995 & -0.8 & 60.3 & 57.7 & 35.7 \\
5650.71 & 26.0 & 5.09 & -0.86 & 68.3 & 64.7 & 39.1 \\
5651.469 & 26.0 & 4.473 & -1.75 & 41.9 & 38.4 & 18.3 \\
5653.87 & 26.0 & 4.39 & -1.54 & 63.8 & 62.1 & 37.2 \\
5661.348 & 26.0 & 4.284 & -1.756 & 51.2 & 47.5 & 22.4 \\
5679.023 & 26.0 & 4.652 & -0.75 & 86.8 & 82.6 & 58.9 \\
5696.09 & 26.0 & 4.548 & -1.72 & 31.9 & 29.9 & 13.6 \\
5701.544 & 26.0 & 2.559 & -2.163 & 127.0 & 120.5 & 81.3 \\
5705.464 & 26.0 & 4.301 & -1.355 & 64.6 & 62.3 & 37.9 \\
5717.83 & 26.0 & 4.28 & -1.03 & 93.2 & 89.1 & 62.3 \\
5731.76 & 26.0 & 4.26 & -1.2 & 85.7 & 82.7 & 57.7 \\
5741.85 & 26.0 & 4.26 & -1.672 & 58.5 & 55.1 & 31.7 \\
5752.03 & 26.0 & 4.55 & -1.177 & 82.1 & 77.4 & 54.9 \\
5775.08 & 26.0 & 4.22 & -1.3 & 87.2 & 83.1 & 58.1 \\
5778.453 & 26.0 & 2.588 & -3.44 & 54.1 & 51.6 & 22.0 \\
5784.658 & 26.0 & 3.396 & -2.532 & 57.0 & 52.6 & 25.8 \\
5809.218 & 26.0 & 3.883 & -1.71 & 89.1 & 82.7 & 49.1 \\
5814.81 & 26.0 & 4.28 & -1.87 & 48.8 & 44.2 & 23.6 \\
5837.7 & 26.0 & 4.29 & -2.24 & 26.2 & 23.5 & 10.1 \\
5849.68 & 26.0 & 3.69 & -2.89 & 25.3 & 21.8 & 8.6 \\
5852.22 & 26.0 & 4.55 & -1.23 & 73.2 & 68.4 & 40.3 \\
5855.076 & 26.0 & 4.608 & -1.478 & 46.8 & 43.6 & 22.8 \\
5856.09 & 26.0 & 4.29 & -1.46 & 59.7 & 56.0 & 33.5 \\
5858.78 & 26.0 & 4.22 & -2.16 & 34.7 & 32.3 & 13.3 \\
5859.59 & 26.0 & 4.55 & -0.58 & 104.6 & 98.8 & 71.9 \\
5861.11 & 26.0 & 4.28 & -2.304 & 24.4 & 21.5 & 8.8 \\
5902.47 & 26.0 & 4.59 & -1.71 & 35.7 & 32.0 & 14.0 \\
5905.67 & 26.0 & 4.65 & -0.69 & 88.3 & 83.8 & 58.8 \\
5909.97 & 26.0 & 3.21 & -2.6 & 69.5 & 63.0 & 33.6 \\
5916.25 & 26.0 & 2.45 & -2.99 & 88.6 & 83.3 & 53.4 \\
5927.79 & 26.0 & 4.65 & -0.99 & 67.4 & 64.4 & 42.6 \\
5929.68 & 26.0 & 4.55 & -1.31 & 66.3 & 62.7 & 39.4 \\
5934.65 & 26.0 & 3.93 & -1.07 & 111.2 & 107.1 & 75.0 \\
5956.694 & 26.0 & 0.859 & -4.552 & 88.0 & 82.2 & 50.5 \\
5976.78 & 26.0 & 3.94 & -1.243 & 103.1 & 98.3 & 66.8 \\
5987.065 & 26.0 & 4.795 & -0.212 & 105.6 & 99.5 & 68.2 \\
6003.01 & 26.0 & 3.88 & -1.06 & 126.4 & 119.4 & 83.7 \\
6005.541 & 26.0 & 2.588 & -3.43 & 58.2 & 52.1 & 22.1 \\
6027.05 & 26.0 & 4.076 & -1.09 & 87.9 & 84.6 & 63.8 \\
6054.07 & 26.0 & 4.37 & -2.333 & 26.7 & 23.7 & 8.4 \\
6056.0 & 26.0 & 4.73 & -0.4 & 103.9 & 97.9 & 71.1 \\
6078.49 & 26.0 & 4.8 & -0.321 & 111.9 & 104.4 & 76.6 \\
6079.01 & 26.0 & 4.65 & -1.02 & 71.9 & 68.8 & 45.3 \\
6082.71 & 26.0 & 2.22 & -3.57 & 70.7 & 64.7 & 35.1 \\
6085.26 & 26.0 & 2.76 & -3.05 & 87.5 & 80.4 & 43.2 \\
6127.91 & 26.0 & 4.14 & -1.4 & 77.0 & 73.4 & 48.1 \\
6151.618 & 26.0 & 2.176 & -3.282 & 82.5 & 77.7 & 49.2 \\
6157.72 & 26.0 & 4.07 & -1.2 & 89.2 & 85.0 & 60.5 \\
6165.36 & 26.0 & 4.143 & -1.46 & 70.0 & 66.1 & 44.3 \\
6173.335 & 26.0 & 2.223 & -2.88 & 102.5 & 97.8 & 67.2 \\
6180.2 & 26.0 & 2.73 & -2.63 & 93.8 & 88.5 & 55.1 \\
6187.99 & 26.0 & 3.94 & -1.62 & 81.5 & 78.2 & 47.7 \\
6200.313 & 26.0 & 2.609 & -2.416 & 110.5 & 105.3 & 71.0 \\
6213.43 & 26.0 & 2.223 & -2.52 & 120.5 & 115.4 & 83.0 \\
6219.28 & 26.0 & 2.2 & -2.43 & 134.5 & 127.5 & 91.0 \\
6226.736 & 26.0 & 3.883 & -2.1 & 60.3 & 55.0 & 29.1 \\
6229.23 & 26.0 & 2.85 & -2.83 & 72.7 & 68.3 & 39.6 \\
6232.64 & 26.0 & 3.65 & -1.22 & 126.6 & 120.3 & 83.9 \\
6240.646 & 26.0 & 2.223 & -3.287 & 77.7 & 73.7 & 48.5 \\
6265.134 & 26.0 & 2.176 & -2.547 & 129.1 & 122.5 & 84.9 \\
6270.225 & 26.0 & 2.858 & -2.54 & 84.8 & 81.2 & 51.1 \\
6271.279 & 26.0 & 3.332 & -2.703 & 56.2 & 51.9 & 23.3 \\
6297.793 & 26.0 & 2.223 & -2.715 & 111.1 & 104.6 & 73.3 \\
6322.69 & 26.0 & 2.59 & -2.43 & 116.7 & 111.6 & 75.9 \\
6335.33 & 26.0 & 2.2 & -2.26 & 138.8 & 132.5 & 96.6 \\
6344.15 & 26.0 & 2.43 & -2.92 & 93.6 & 89.5 & 59.0 \\
6358.68 & 26.0 & 0.86 & -4.24 & 134.1 & 128.8 & 83.7 \\
6380.74 & 26.0 & 4.19 & -1.32 & 80.9 & 78.5 & 51.5 \\
6392.539 & 26.0 & 2.279 & -4.03 & 48.4 & 42.9 & 16.8 \\
6419.95 & 26.0 & 4.73 & -0.24 & 124.9 & 120.0 & 76.9 \\
6430.846 & 26.0 & 2.176 & -2.006 & 172.3 & 163.3 & 111.0 \\
6481.87 & 26.0 & 2.28 & -2.98 & 101.8 & 95.2 & 64.8 \\
6498.939 & 26.0 & 0.958 & -4.695 & 85.9 & 81.0 & 45.6 \\
6518.367 & 26.0 & 2.831 & -2.448 & 91.5 & 86.1 & 56.5 \\
6574.229 & 26.0 & 0.99 & -5.01 & 70.8 & 65.5 & 28.5 \\
6593.871 & 26.0 & 2.433 & -2.394 & 124.1 & 116.9 & 83.7 \\
6597.56 & 26.0 & 4.8 & -0.97 & 72.1 & 68.2 & 43.7 \\
6609.11 & 26.0 & 2.559 & -2.682 & 96.4 & 92.0 & 65.7 \\
6699.142 & 26.0 & 4.593 & -2.101 & 24.8 & 23.1 & 8.3 \\
6625.022 & 26.0 & 1.011 & -5.336 & 53.7 & 49.2 & 15.0 \\
6703.567 & 26.0 & 2.759 & -3.023 & 72.1 & 68.4 & 36.6 \\
6705.102 & 26.0 & 4.607 & -0.98 & 79.7 & 75.4 & 46.4 \\
6710.319 & 26.0 & 1.485 & -4.88 & 52.9 & 47.5 & 15.7 \\
6713.745 & 26.0 & 4.795 & -1.4 & 44.7 & 42.1 & 21.2 \\
6725.357 & 26.0 & 4.103 & -2.19 & 43.1 & 39.6 & 18.3 \\
6726.667 & 26.0 & 4.607 & -1.03 & 76.7 & 72.8 & 46.2 \\
6733.151 & 26.0 & 4.638 & -1.47 & 53.4 & 50.7 & 26.6 \\
6739.522 & 26.0 & 1.557 & -4.794 & 41.9 & 37.2 & 11.4 \\
6750.152 & 26.0 & 2.424 & -2.621 & 111.7 & 108.0 & 73.5 \\
6806.845 & 26.0 & 2.727 & -3.11 & 70.3 & 65.0 & 35.0 \\
6810.263 & 26.0 & 4.607 & -0.986 & 79.7 & 76.6 & 49.9 \\
6828.59 & 26.0 & 4.64 & -0.82 & 86.5 & 82.3 & 54.8 \\
6837.006 & 26.0 & 4.593 & -1.687 & 38.8 & 35.0 & 17.0 \\
6839.83 & 26.0 & 2.559 & -3.35 & 66.5 & 61.5 & 30.5 \\
6841.34 & 26.0 & 4.61 & -0.71 & 85.1 & 80.5 & 60.8 \\
6842.69 & 26.0 & 4.64 & -1.22 & 66.8 & 62.7 & 38.3 \\
6843.66 & 26.0 & 4.55 & -0.83 & 94.6 & 89.6 & 60.8 \\
6854.823 & 26.0 & 4.593 & -1.926 & 30.8 & 27.8 & 12.9 \\
6855.16 & 26.0 & 4.56 & -0.74 & 104.6 & 101.5 & 71.9 \\
6858.15 & 26.0 & 4.61 & -0.94 & 79.6 & 74.8 & 51.3 \\
7090.38 & 26.0 & 4.23 & -1.11 & 110.0 & 103.3 & 66.3 \\
7132.99 & 26.0 & 4.08 & -1.65 & 72.1 & 68.7 & 42.5 \\
7401.685 & 26.0 & 4.186 & -1.5 & 67.9 & 64.7 & 41.7 \\
7418.67 & 26.0 & 4.14 & -1.38 & 80.2 & 75.4 & 48.9 \\
7583.79 & 26.0 & 3.02 & -1.88 & 126.4 & 119.9 & 82.8 \\
7710.36 & 26.0 & 4.22 & -1.11 & 105.0 & 100.7 & 67.0 \\
7723.21 & 26.0 & 2.28 & -3.62 & 82.0 & 74.7 & 40.6 \\
4508.29 & 26.1 & 2.856 & -2.52 & 85.2 & 84.4 & 84.7 \\
4520.224 & 26.1 & 2.8068 & -2.65 & 76.3 & 75.7 & 78.6 \\
4576.333 & 26.1 & 2.844 & -2.95 & 69.1 & 69.6 & 64.4 \\
4993.34 & 26.1 & 2.81 & -3.73 & 46.1 & 45.2 & 39.1 \\
5197.577 & 26.1 & 3.231 & -2.22 & 81.0 & 81.3 & 88.4 \\
5234.624 & 26.1 & 3.221 & -2.18 & 81.1 & 81.3 & 82.4 \\
5264.804 & 26.1 & 3.23 & -3.13 & 44.6 & 44.4 & 45.1 \\
5414.072 & 26.1 & 3.221 & -3.58 & 29.7 & 29.8 & 26.7 \\
5425.257 & 26.1 & 3.2 & -3.22 & 44.8 & 46.0 & 41.1 \\
5534.84 & 26.1 & 3.24 & -2.88 & 57.6 & 57.6 & 56.0 \\
6084.09 & 26.1 & 3.2 & -3.83 & 24.8 & 24.4 & 21.3 \\
6149.24 & 26.1 & 3.89 & -2.75 & 35.8 & 35.7 & 34.9 \\
6238.38 & 26.1 & 3.89 & -2.63 & 49.7 & 48.3 & 44.3 \\
6247.55 & 26.1 & 3.89 & -2.38 & 49.6 & 49.1 & 54.1 \\
6369.462 & 26.1 & 2.891 & -4.11 & 19.9 & 20.6 & 18.6 \\
6432.676 & 26.1 & 2.891 & -3.57 & 42.3 & 41.7 & 40.9 \\
6456.383 & 26.1 & 3.9036 & -2.05 & 56.6 & 56.8 & 61.0 \\
6516.077 & 26.1 & 2.891 & -3.31 & 59.4 & 60.7 & 56.3 \\
7711.721 & 26.1 & 3.903 & -2.5 & 47.0 & 46.7 & 46.2 \\

